Can Large Language Models Adequately Perform Symbolic Reasoning Over Time Series?

Uncovering hidden symbolic laws from time series data, as an aspiration dating back to Kepler's discovery of planetary motion, remains a core challenge in scientific discovery and artificial intelligence. While Large Language Models show promise in structured reasoning tasks, their ability to infer interpretable, context-aligned symbolic structures from time series data is still underexplored. To systematically evaluate this capability, we introduce SymbolBench, a comprehensive benchmark designed to assess symbolic reasoning over real-world time series across three tasks: multivariate symbolic regression, Boolean network inference, and causal discovery. Unlike prior efforts limited to simple algebraic equations, SymbolBench spans a diverse set of symbolic forms with varying complexity. We further propose a unified framework that integrates LLMs with genetic programming to form a closed-loop symbolic reasoning system, where LLMs act both as predictors and evaluators. Our empirical results reveal key strengths and limitations of current models, highlighting the importance of combining domain knowledge, context alignment, and reasoning structure to improve LLMs in automated scientific discovery. https://github.com/nuuuh/SymbolBench.

==> sections/raw_datasets.tex <==
\section{Coupled Differential Equations Dataset}
\label{appendix: coupled_DEs}








\clearpage
\section{Boolean Networks Dataset}
\label{appendix: BNs}

% \begin{longtable}[ht]      
% \footnotesize                     % or \scriptsize if you need a bit more room
% \centering
% \renewcommand{\arraystretch}{1.1}  % tighter vertical padding

% % Scale to textheight (the longer A4 edge) so nothing spills
% \resizebox{0.8\textheight}{!}{%
%   \begin{tabular}{
%     p{4cm}    % model_name  – wraps in 4 cm
%     >{\centering\arraybackslash}p{0.1cm}  % num_var
%     >{\centering\arraybackslash}p{0.4cm}    % num_inputs
%     >{\centering\arraybackslash}p{0.8cm}  % num_regulars
%     p{4.5cm} % variable_mapping – wraps
%     p{7.5cm} % regulations      – wraps
%   }

\footnotesize
%\begin{adjustbox}{max width=\linewidth,center}  % enable if you need it
\begin{longtable}{
  p{1cm} >{\centering\arraybackslash}p{0.9cm}
  >{\centering\arraybackslash}p{0.3cm} >{\centering\arraybackslash}p{1cm}
  p{3cm} p{7.5cm}}
\caption{Boolean‑network models used in this study}\label{tab:bn-summary}\\

\toprule
model\_name & var & inputs & regulars & variable\_mapping & regulations \\
\midrule
DROSOPHILA-WINGS-AP & 10 & 2 & 8 & x1: v\_Ap, x2: v\_Ap2, x3: v\_Dl, x4: v\_Dl2, x5: v\_Fng, x6: v\_Fng2, x7: v\_N, x8: v\_N2, x9: v\_Ser, x10: v\_Ser2 & x3 = ( NOT x1 AND x7 )
x4 = ( NOT x2 AND x8 )
x5 = x1
x6 = x2
x7 = ( ( NOT x5 AND x10 ) OR ( x5 AND x4 ) )
x8 = ( ( ( ( NOT x3 AND x9 ) AND NOT x6 ) OR ( ( x3 AND NOT x9 ) AND x6 ) ) OR ( x3 AND x9 ) )
x9 = x1
x10 = x2 \\
LAMBDA-PHAGE-LYSOGENY & 7 & 0 & 7 & x1: v\_CII, x2: v\_CI\_b1, x3: v\_CI\_b2, x4: v\_Cro\_b1, x5: v\_Cro\_b2, x6: v\_Cro\_b3, x7: v\_N & x1 = ( ( ( ( ( ( ( NOT x2 AND NOT x4 ) AND x7 ) OR ( ( ( NOT x2 AND x4 ) AND NOT x5 ) AND x7 ) ) OR ( ( ( ( NOT x2 AND x4 ) AND x5 ) AND NOT x6 ) AND x7 ) ) OR ( ( ( x2 AND NOT x3 ) AND NOT x4 ) AND x7 ) ) OR ( ( ( ( x2 AND NOT x3 ) AND x4 ) AND NOT x5 ) AND x7 ) ) OR ( ( ( ( ( x2 AND NOT x3 ) AND x4 ) AND x5 ) AND NOT x6 ) AND x7 ) )
x2 = ( ( ( ( ( NOT x2 AND NOT x4 ) OR ( ( NOT x2 AND x4 ) AND x1 ) ) OR ( ( x2 AND NOT x3 ) AND NOT x4 ) ) OR ( ( ( x2 AND NOT x3 ) AND x4 ) AND x1 ) ) OR ( x2 AND x3 ) )
x3 = ( ( x2 AND NOT x4 ) OR ( ( x2 AND x4 ) AND x1 ) )
x4 = ( ( NOT x2 OR ( x2 AND NOT x3 ) ) OR ( ( ( x2 AND x3 ) AND x4 ) AND x5 ) )
x5 = ( ( ( NOT x2 AND x4 ) OR ( ( x2 AND NOT x3 ) AND x4 ) ) OR ( ( ( ( x2 AND x3 ) AND x4 ) AND x5 ) AND x6 ) )
x6 = ( ( ( ( NOT x2 AND x4 ) AND x5 ) AND NOT x6 ) OR ( ( ( ( x2 AND NOT x3 ) AND x4 ) AND x5 ) AND NOT x6 ) )
x7 = ( ( NOT x2 AND NOT x4 ) OR ( ( NOT x2 AND x4 ) AND NOT x5 ) ) \\
PREDICTING-VARIABILITIES-IN-CARDIAC-GENE & 15 & 2 & 13 & x1: v\_Bmp2, x2: v\_Dkk1, x3: v\_Fgf8, x4: v\_Foxc1\_2, x5: v\_GATAs, x6: v\_Isl1, x7: v\_Mesp1\_, x8: v\_Nkx2\_5\_, x9: v\_Tbx1, x10: v\_Tbx5, x11: v\_canWnt, x12: v\_exogen\_BMP2\_I, x13: v\_exogen\_BMP2\_II, x14: v\_exogen\_CanWnt\_I, x15: v\_exogen\_CanWnt\_II & x1 = ( x13 AND NOT x11 )
x2 = ( ( x11 AND NOT x13 ) OR x7 )
x3 = ( ( x9 AND NOT x7 ) OR ( x4 AND NOT x7 ) )
x4 = ( x11 AND x15 )
x5 = ( ( x7 OR x8 ) OR x10 )
x6 = ( ( ( x7 OR x9 ) OR ( x11 AND x15 ) ) OR x3 )
x7 = ( x11 AND NOT x13 )
x8 = ( ( ( ( x10 OR ( x5 AND x1 ) ) OR ( x6 AND x5 ) ) OR x9 ) OR ( x7 AND x2 ) )
x9 = x4
x10 = ( ( ( x10 AND NOT ( ( x9 OR ( x2 AND ( NOT x10 AND NOT x7 ) ) ) OR x11 ) ) OR ( x7 AND NOT ( ( x9 OR ( x2 AND ( NOT x10 AND NOT x7 ) ) ) OR x11 ) ) ) OR ( x8 AND NOT ( ( x9 OR ( x2 AND ( NOT x10 AND NOT x7 ) ) ) OR x11 ) ) )
x11 = x15
x13 = x12
x15 = x14 \\
HCC1954-BREAST-CELL-LINE-SHORT-TERM & 16 & 5 & 11 & x1: v\_AKT, x2: v\_EGF, x3: v\_ERBB1, x4: v\_ERBB2, x5: v\_ERBB3, x6: v\_ERK1\_2, x7: v\_HRG, x8: v\_MEK1\_2, x9: v\_PDK1, x10: v\_PKCa, x11: v\_PLCg, x12: v\_erlotinib, x13: v\_mTOR, x14: v\_p70S6K, x15: v\_pertuzumab, x16: v\_trastuzumab & x1 = ( ( ( ( x14 OR x13 ) OR x5 ) OR x9 ) OR x1 )
x3 = ( ( ( x2 AND NOT ( x15 OR x12 ) ) OR ( x3 AND NOT ( x15 OR x12 ) ) ) OR ( x11 AND NOT ( x15 OR x12 ) ) )
x4 = ( ( ( x3 AND NOT ( ( x12 OR x16 ) OR x15 ) ) OR ( x4 AND NOT ( ( x12 OR x16 ) OR x15 ) ) ) OR ( x9 AND NOT ( ( x12 OR x16 ) OR x15 ) ) )
x5 = ( ( ( x6 AND NOT ( x12 OR x15 ) ) OR ( x5 AND NOT ( x12 OR x15 ) ) ) OR ( x7 AND NOT ( x12 OR x15 ) ) )
x6 = ( x8 OR x6 )
x8 = ( ( ( ( x3 OR x9 ) OR x8 ) OR x4 ) OR x5 )
x9 = ( ( ( x4 OR x9 ) OR x3 ) OR x5 )
x10 = ( ( x11 OR x10 ) OR x16 )
x11 = ( ( ( x3 OR x4 ) OR x11 ) OR x5 )
x13 = ( x1 OR x13 )
x14 = ( ( ( ( x13 OR x12 ) OR x14 ) OR x1 ) OR x6 ) \\
CHICKEN-SEX-DETERMINATION-REDUCED & 10 & 3 & 7 & x1: v\_AROMATASE, x2: v\_DMRT1\_b1, x3: v\_DMRT1\_b2, x4: v\_FOXL2, x5: v\_HEMGN, x6: v\_OESTROGEN, x7: v\_SOX9, x8: v\_W, x9: v\_Z1, x10: v\_Z2 & x1 = ( ( NOT x4 AND x6 ) OR x4 )
x2 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x9 AND NOT x2 ) AND NOT x5 ) AND x7 ) AND NOT x4 ) OR ( ( ( NOT x9 AND NOT x2 ) AND x5 ) AND NOT x4 ) ) OR ( ( ( ( ( NOT x9 AND x2 ) AND NOT x3 ) AND NOT x5 ) AND x7 ) AND NOT x4 ) ) OR ( ( ( ( NOT x9 AND x2 ) AND NOT x3 ) AND x5 ) AND NOT x4 ) ) OR ( ( NOT x9 AND x2 ) AND x3 ) ) OR ( ( ( ( ( x9 AND NOT x10 ) AND NOT x2 ) AND NOT x5 ) AND x7 ) AND NOT x4 ) ) OR ( ( ( ( x9 AND NOT x10 ) AND NOT x2 ) AND x5 ) AND NOT x4 ) ) OR ( ( ( ( ( ( x9 AND NOT x10 ) AND x2 ) AND NOT x3 ) AND NOT x5 ) AND x7 ) AND NOT x4 ) ) OR ( ( ( ( ( x9 AND NOT x10 ) AND x2 ) AND NOT x3 ) AND x5 ) AND NOT x4 ) ) OR ( ( ( x9 AND NOT x10 ) AND x2 ) AND x3 ) ) OR ( ( ( ( x9 AND x10 ) AND NOT x8 ) AND NOT x2 ) AND NOT x4 ) ) OR ( ( ( ( ( x9 AND x10 ) AND NOT x8 ) AND x2 ) AND NOT x3 ) AND NOT x4 ) ) OR ( ( ( ( x9 AND x10 ) AND NOT x8 ) AND x2 ) AND x3 ) ) OR ( ( ( ( ( ( x9 AND x10 ) AND x8 ) AND NOT x2 ) AND NOT x5 ) AND x7 ) AND NOT x4 ) ) OR ( ( ( ( ( x9 AND x10 ) AND x8 ) AND NOT x2 ) AND x5 ) AND NOT x4 ) ) OR ( ( ( ( ( ( ( x9 AND x10 ) AND x8 ) AND x2 ) AND NOT x3 ) AND NOT x5 ) AND x7 ) AND NOT x4 ) ) OR ( ( ( ( ( ( x9 AND x10 ) AND x8 ) AND x2 ) AND NOT x3 ) AND x5 ) AND NOT x4 ) ) OR ( ( ( ( x9 AND x10 ) AND x8 ) AND x2 ) AND x3 ) )
x3 = ( ( ( ( x2 AND NOT x5 ) AND x7 ) AND NOT x4 ) OR ( ( x2 AND x5 ) AND NOT x4 ) )
x4 = ( ( ( ( NOT x2 AND NOT x7 ) OR ( ( NOT x2 AND x7 ) AND x6 ) ) OR ( ( x2 AND NOT x3 ) AND NOT x7 ) ) OR ( ( ( x2 AND NOT x3 ) AND x7 ) AND x6 ) )
x5 = ( x2 AND NOT x7 )
x6 = x1
x7 = ( ( ( ( NOT x2 AND x7 ) AND NOT x4 ) OR ( ( ( x2 AND NOT x3 ) AND x7 ) AND NOT x4 ) ) OR ( ( x2 AND x3 ) AND NOT x4 ) ) \\
MAMMALIAN-CELL-CYCLE-2006 & 10 & 1 & 9 & x1: v\_Cdc20, x2: v\_Cdh1, x3: v\_CycA, x4: v\_CycB, x5: v\_CycD, x6: v\_CycE, x7: v\_E2F, x8: v\_Rb, x9: v\_UbcH10, x10: v\_p27 & x1 = x4
x2 = ( ( x1 OR ( x10 AND NOT x4 ) ) OR NOT ( ( ( x10 OR x4 ) OR x3 ) OR x1 ) )
x3 = ( ( x3 AND NOT ( ( ( x2 AND x9 ) OR x1 ) OR x8 ) ) OR ( x7 AND NOT ( ( ( x2 AND x9 ) OR x1 ) OR x8 ) ) )
x4 = NOT ( x1 OR x2 )
x6 = ( x7 AND NOT x8 )
x7 = ( ( x10 AND NOT ( x4 OR x8 ) ) OR NOT ( ( ( x10 OR x8 ) OR x4 ) OR x3 ) )
x8 = ( ( x10 AND NOT ( x5 OR x4 ) ) OR NOT ( ( ( ( x6 OR x10 ) OR x4 ) OR x5 ) OR x3 ) )
x9 = ( ( ( ( ( x9 AND ( ( x2 AND ( ( x4 OR x1 ) OR x3 ) ) OR NOT x2 ) ) OR ( x3 AND NOT x2 ) ) OR ( x1 AND NOT x2 ) ) OR ( x4 AND NOT x2 ) ) OR NOT ( ( ( ( x9 OR x2 ) OR x4 ) OR x1 ) OR x3 ) )
x10 = ( ( x10 AND NOT ( ( x5 OR ( x3 AND x6 ) ) OR x4 ) ) OR NOT ( ( ( ( x6 OR x10 ) OR x4 ) OR x5 ) OR x3 ) ) \\
MAMMAL-SEX-DETERMINATION-1-CELL & 19 & 6 & 13 & x1: v\_AF, x2: v\_AS, x3: v\_Dmrt1, x4: v\_Fgf9\_b1, x5: v\_Fgf9\_b2, x6: v\_Foxl2, x7: v\_Gata4, x8: v\_IW, x9: v\_Sf1\_b1, x10: v\_Sf1\_b2, x11: v\_Sox9\_b1, x12: v\_Sox9\_b2, x13: v\_Sry, x14: v\_Wnt4\_b1, x15: v\_Wnt4\_b2, x16: v\_Wt1, x17: v\_Y, x18: v\_b\_cat\_b1, x19: v\_b\_cat\_b2 & x3 = ( ( ( ( ( NOT x7 AND x9 ) AND x11 ) AND x12 ) AND NOT x6 ) OR ( x7 AND NOT x6 ) )
x4 = ( ( ( NOT x11 AND x4 ) OR ( ( x11 AND NOT x12 ) AND x4 ) ) OR ( x11 AND x12 ) )
x5 = ( ( x11 AND x12 ) AND x4 )
x6 = ( x1 AND NOT x3 )
x9 = ( ( ( NOT x16 AND x9 ) AND x10 ) OR x16 )
x10 = ( ( ( x16 AND x9 ) AND x11 ) AND x12 )
x11 = ( ( ( ( ( ( ( NOT x9 AND x11 ) AND x12 ) OR ( ( ( x9 AND NOT x11 ) AND NOT x18 ) AND NOT x6 ) ) OR ( ( ( ( x9 AND NOT x11 ) AND x18 ) AND NOT x19 ) AND NOT x6 ) ) OR ( ( ( ( x9 AND x11 ) AND NOT x12 ) AND NOT x18 ) AND NOT x6 ) ) OR ( ( ( ( ( x9 AND x11 ) AND NOT x12 ) AND x18 ) AND NOT x19 ) AND NOT x6 ) ) OR ( ( x9 AND x11 ) AND x12 ) )
x12 = ( ( ( ( ( ( NOT x13 AND x9 ) AND x11 ) AND NOT x18 ) AND NOT x6 ) OR ( ( ( ( x13 AND x9 ) AND x11 ) AND NOT x18 ) AND NOT x6 ) ) OR ( ( ( ( ( x13 AND x9 ) AND x11 ) AND x18 ) AND NOT x19 ) AND NOT x6 ) )
x13 = ( ( ( ( ( ( x17 AND x16 ) AND x2 ) AND x7 ) AND x9 ) AND NOT x11 ) OR ( ( ( ( ( ( x17 AND x16 ) AND x2 ) AND x7 ) AND x9 ) AND x11 ) AND NOT x12 ) )
x14 = ( ( NOT x8 AND x14 ) OR ( ( x8 AND x14 ) AND x15 ) )
x15 = ( ( NOT x8 AND NOT x4 ) AND x14 )
x18 = ( ( ( ( ( ( ( NOT x11 AND NOT x14 ) AND x18 ) AND x19 ) OR ( NOT x11 AND x14 ) ) OR ( ( ( ( x11 AND NOT x12 ) AND NOT x14 ) AND x18 ) AND x19 ) ) OR ( ( x11 AND NOT x12 ) AND x14 ) ) OR ( ( ( x11 AND x12 ) AND x18 ) AND x19 ) )
x19 = ( ( ( ( NOT x11 AND x14 ) AND x15 ) AND x18 ) OR ( ( ( ( x11 AND NOT x12 ) AND x14 ) AND x15 ) AND x18 ) ) \\
ESCHERICHIA-COLI-TRYPTOPHAN & 16 & 3 & 13 & x1: v\_A, x2: v\_B, x3: v\_C, x4: v\_E, x5: v\_E\_m, x6: v\_L, x7: v\_M\_1, x8: v\_M\_2, x9: v\_P, x10: v\_R, x11: v\_T, x12: v\_W, x13: v\_W\_m, x14: v\_gamma, x15: v\_omega\_e, x16: v\_omega\_em & x1 = ( x8 AND NOT x14 )
x2 = x8
x3 = NOT x14
x4 = ( x7 AND NOT x6 )
x5 = ( x7 OR x4 )
x6 = ( x7 AND x11 )
x7 = NOT x10
x8 = ( x3 AND NOT x9 )
x9 = ( NOT x12 AND NOT x13 )
x10 = x12
x11 = x13
x12 = ( ( x7 AND ( NOT x6 AND NOT x1 ) ) OR ( x15 AND x2 ) )
x13 = ( x7 OR ( x12 OR ( x15 OR ( x16 AND x2 ) ) ) ) \\
SKBR3-BREAST-CELL-LINE-SHORT-TERM & 16 & 5 & 11 & x1: v\_AKT, x2: v\_EGF, x3: v\_ERBB1, x4: v\_ERBB2, x5: v\_ERBB3, x6: v\_ERK1\_2, x7: v\_HRG, x8: v\_MEK1\_2, x9: v\_PDK1, x10: v\_PKCa, x11: v\_PLCg, x12: v\_erlotinib, x13: v\_mTOR, x14: v\_p70S6K, x15: v\_pertuzumab, x16: v\_trastuzumab & x1 = ( ( ( x13 OR x9 ) OR x1 ) OR x5 )
x3 = ( ( ( x3 AND NOT ( x15 OR x12 ) ) OR ( x2 AND NOT ( x15 OR x12 ) ) ) OR ( x11 AND NOT ( x15 OR x12 ) ) )
x4 = ( x4 AND NOT ( ( x16 OR x15 ) OR x12 ) )
x5 = ( ( x5 AND NOT ( x12 OR x15 ) ) OR ( x7 AND NOT ( x12 OR x15 ) ) )
x6 = ( ( ( x9 OR x5 ) OR x8 ) OR x6 )
x8 = ( ( ( x4 OR x5 ) OR x3 ) OR x8 )
x9 = ( ( ( x4 OR x3 ) OR x9 ) OR x5 )
x10 = ( x11 OR x10 )
x11 = ( ( ( x4 OR x5 ) OR x3 ) OR x11 )
x13 = ( x13 OR x1 )
x14 = ( ( ( x14 OR x1 ) OR x13 ) OR x6 ) \\
MAPK-REDUCED-2 & 18 & 4 & 14 & x1: v\_AKT, x2: v\_Apoptosis, x3: v\_DNA\_damage, x4: v\_EGFR, x5: v\_EGFR\_stimulus, x6: v\_ERK, x7: v\_FGFR3, x8: v\_FGFR3\_stimulus, x9: v\_GRB2, x10: v\_Growth\_Arrest, x11: v\_PI3K, x12: v\_Proliferation, x13: v\_RAF, x14: v\_RAS, x15: v\_TGFBR\_stimulus, x16: v\_p21, x17: v\_p38, x18: v\_p53 & x1 = ( NOT x18 AND x11 )
x2 = ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND x18 ) AND NOT x1 ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND x18 ) AND NOT x1 ) AND x14 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND x18 ) AND NOT x1 ) ) OR ( ( ( x15 AND NOT x6 ) AND x18 ) AND NOT x1 ) )
x4 = ( ( ( ( ( NOT x5 AND x6 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) OR ( ( ( x5 AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) )
x6 = ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x18 ) AND x13 ) AND NOT x14 ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND NOT x18 ) AND NOT x13 ) AND x14 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND NOT x18 ) AND x13 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND x18 ) AND x13 ) AND NOT x14 ) ) OR ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x18 ) AND x13 ) AND NOT x14 ) )
x7 = ( ( ( x8 AND NOT x4 ) AND NOT x7 ) AND NOT x9 )
x9 = ( ( ( ( ( ( ( NOT x15 AND NOT x6 ) AND NOT x4 ) AND x7 ) AND NOT x9 ) OR ( ( NOT x15 AND NOT x6 ) AND x4 ) ) OR ( ( NOT x15 AND x6 ) AND x4 ) ) OR x15 )
x10 = x16
x11 = ( ( NOT x9 AND x11 ) OR x9 )
x12 = ( ( ( ( ( x6 AND NOT x17 ) AND NOT x16 ) AND x1 ) AND x11 ) OR ( ( ( x6 AND x17 ) AND NOT x16 ) AND x11 ) )
x13 = ( ( ( ( ( ( NOT x6 AND NOT x4 ) AND NOT x7 ) AND NOT x1 ) AND x14 ) OR ( ( ( NOT x6 AND NOT x4 ) AND x7 ) AND NOT x1 ) ) OR ( ( NOT x6 AND x4 ) AND NOT x1 ) )
x14 = ( ( ( ( ( ( ( NOT x6 AND NOT x4 ) AND NOT x7 ) AND x9 ) OR ( ( NOT x6 AND NOT x4 ) AND x7 ) ) OR ( NOT x6 AND x4 ) ) OR ( ( x6 AND NOT x4 ) AND x7 ) ) OR ( x6 AND x4 ) )
x16 = ( x18 AND NOT x1 )
x17 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x18 ) AND x14 ) OR ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND x18 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND x18 ) AND x14 ) ) OR ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND x18 ) AND x14 ) ) OR ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) ) OR ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND x17 ) AND NOT x18 ) AND x14 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND x17 ) AND x18 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x18 ) AND x14 ) ) OR ( ( ( NOT x15 AND x3 ) AND x6 ) AND x18 ) ) OR x15 )
x18 = ( ( ( ( ( ( NOT x3 AND x17 ) OR ( ( ( ( x3 AND NOT x6 ) AND NOT x17 ) AND NOT x18 ) AND NOT x1 ) ) OR ( ( x3 AND NOT x6 ) AND x17 ) ) OR ( ( ( x3 AND x6 ) AND NOT x17 ) AND NOT x18 ) ) OR ( ( ( ( x3 AND x6 ) AND NOT x17 ) AND x18 ) AND x1 ) ) OR ( ( x3 AND x6 ) AND x17 ) ) \\
ASYMMETRIC-CELL-DIVISION-B & 9 & 0 & 9 & x1: v\_CckA, x2: v\_ChpT, x3: v\_ClpXP\_RcdA, x4: v\_CpdR, x5: v\_CtrAb, x6: v\_DivJ, x7: v\_DivK, x8: v\_DivL, x9: v\_PleC & x1 = x8
x2 = x1
x3 = NOT x4
x4 = x2
x5 = ( x2 AND NOT x3 )
x6 = ( x7 AND NOT x9 )
x7 = ( NOT x9 AND x6 )
x8 = NOT x7
x9 = NOT x7 \\
T-LGL-SURVIVAL-NETWORK-2011-REDUCED & 18 & 0 & 18 & x1: v\_Apoptosis\_, x2: v\_BID\_, x3: v\_CREB, x4: v\_CTLA4\_, x5: v\_Caspase, x6: v\_Ceramide\_, x7: v\_DISC\_, x8: v\_FLIP\_, x9: v\_Fas, x10: v\_GPCR\_, x11: v\_IAP\_, x12: v\_IFNG\_, x13: v\_MCL1, x14: v\_P2, x15: v\_S1P, x16: v\_SMAD\_, x17: v\_TCR, x18: v\_sFas & x1 = ( x5 OR x1 )
x2 = NOT ( x13 OR x1 )
x3 = ( x12 AND NOT x1 )
x4 = ( x17 AND NOT x1 )
x5 = ( ( x2 AND NOT ( x11 OR x1 ) ) OR ( x7 AND NOT x1 ) )
x6 = ( x9 AND NOT ( x1 OR x15 ) )
x7 = ( ( x9 AND NOT ( x8 OR x1 ) ) OR ( x6 AND NOT x1 ) )
x8 = NOT ( x1 OR x7 )
x9 = NOT ( x1 OR x18 )
x10 = ( x15 AND NOT x1 )
x11 = NOT ( x2 OR x1 )
x12 = NOT ( ( x14 OR x1 ) OR x16 )
x13 = NOT ( x1 OR x7 )
x14 = ( ( x12 AND NOT x1 ) OR ( x14 AND NOT x1 ) )
x15 = NOT ( x1 OR x6 )
x16 = ( x10 AND NOT x1 )
x17 = NOT ( x1 OR x4 )
x18 = ( x15 AND NOT x1 ) \\
YEAST-HYPHAL-TRANSITION & 19 & 3 & 16 & x1: v\_Brg1, x2: v\_Cyr1, x3: v\_EFG1\_T, x4: v\_ESCRT, x5: v\_Efg1, x6: v\_Efg1\_active, x7: v\_Farnesol, x8: v\_HAG\_T, x9: v\_HATs, x10: v\_HDACs, x11: v\_NRG1\_T, x12: v\_Nrg1\_HAGs, x13: v\_Rim8, x14: v\_Temperature, x15: v\_Ume6, x16: v\_cAMP\_PKA, x17: v\_hyphal\_initiation, x18: v\_hyphal\_maintenance, x19: v\_pH & x1 = NOT x12
x2 = ( NOT x7 AND x14 )
x3 = ( NOT x6 OR ( x6 AND x1 ) )
x4 = x13
x5 = x3
x6 = ( ( ( NOT x4 AND x16 ) AND x5 ) OR ( x4 AND x5 ) )
x8 = ( ( ( NOT x12 AND NOT x1 ) AND x15 ) OR ( NOT x12 AND x1 ) )
x9 = ( x6 AND NOT x10 )
x10 = x1
x11 = ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x4 AND NOT x16 ) AND NOT x1 ) AND NOT x15 ) OR ( ( ( ( NOT x4 AND NOT x16 ) AND NOT x1 ) AND x15 ) AND x17 ) ) OR ( ( ( NOT x4 AND NOT x16 ) AND x1 ) AND x17 ) ) OR ( ( ( ( NOT x4 AND x16 ) AND NOT x6 ) AND NOT x1 ) AND NOT x15 ) ) OR ( ( ( ( ( NOT x4 AND x16 ) AND NOT x6 ) AND NOT x1 ) AND x15 ) AND x17 ) ) OR ( ( ( ( NOT x4 AND x16 ) AND NOT x6 ) AND x1 ) AND x17 ) ) OR ( ( ( NOT x4 AND x16 ) AND x6 ) AND x17 ) ) OR ( ( ( x4 AND NOT x6 ) AND NOT x1 ) AND NOT x15 ) ) OR ( ( ( ( x4 AND NOT x6 ) AND NOT x1 ) AND x15 ) AND x17 ) ) OR ( ( ( x4 AND NOT x6 ) AND x1 ) AND x17 ) ) OR ( ( x4 AND x6 ) AND x17 ) )
x12 = ( ( x11 AND NOT x10 ) OR ( ( x11 AND x10 ) AND x9 ) )
x13 = x19
x15 = ( NOT x12 AND x1 )
x16 = x2
x17 = ( ( ( ( ( NOT x12 AND NOT x1 ) AND x17 ) OR ( ( ( NOT x12 AND x1 ) AND NOT x9 ) AND x17 ) ) OR ( ( NOT x12 AND x1 ) AND x9 ) ) OR ( x12 AND x17 ) )
x18 = ( ( NOT x12 AND x15 ) AND x17 ) \\
DROSOPHILA-GAP-C & 7 & 2 & 5 & x1: v\_Gt, x2: v\_Hb\_b1, x3: v\_Hb\_b2, x4: v\_Hb\_b3, x5: v\_Kni, x6: v\_Kr\_b1, x7: v\_Kr\_b2 & x1 = NOT x6
x3 = ( ( x2 AND x3 ) AND x4 )
x5 = ( ( NOT x1 AND NOT x2 ) OR ( ( NOT x1 AND x2 ) AND NOT x3 ) )
x6 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x1 AND NOT x2 ) AND x6 ) AND x7 ) OR ( ( NOT x1 AND x2 ) AND NOT x3 ) ) OR ( ( ( NOT x1 AND x2 ) AND x3 ) AND NOT x4 ) ) OR ( ( ( ( ( NOT x1 AND x2 ) AND x3 ) AND x4 ) AND x6 ) AND x7 ) ) OR ( ( ( x1 AND NOT x2 ) AND x6 ) AND x7 ) ) OR ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND NOT x6 ) AND NOT x5 ) ) OR ( ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND x6 ) AND NOT x7 ) AND NOT x5 ) ) OR ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND x6 ) AND x7 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND NOT x6 ) AND NOT x5 ) ) OR ( ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND NOT x7 ) AND NOT x5 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND x7 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND x4 ) AND x6 ) AND x7 ) )
x7 = ( ( ( ( ( NOT x1 AND x2 ) AND NOT x3 ) AND x6 ) AND NOT x5 ) OR ( ( ( ( ( NOT x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND NOT x5 ) ) \\
CONTROL-OF-PROLIFERATION & 18 & 1 & 17 & x1: v\_AKT, x2: v\_E2F, x3: v\_EIF4F, x4: v\_FOXO3, x5: v\_GFs, x6: v\_MAPK, x7: v\_PI3K, x8: v\_PIP3, x9: v\_PRAS40, x10: v\_Proliferation\_b1, x11: v\_Proliferation\_b2, x12: v\_RAS, x13: v\_RTK, x14: v\_Rb, x15: v\_S6K, x16: v\_TSC, x17: v\_cycE, x18: v\_mTORC1 & x1 = x8
x2 = NOT x14
x3 = x18
x4 = ( NOT x6 OR ( x6 AND NOT x1 ) )
x6 = ( ( NOT x12 AND x8 ) OR x12 )
x7 = ( ( NOT x13 AND x12 ) OR x13 )
x8 = x7
x9 = NOT x1
x10 = ( ( ( ( ( ( NOT x2 AND NOT x3 ) AND x10 ) AND x11 ) OR ( ( ( ( NOT x2 AND x3 ) AND NOT x15 ) AND x10 ) AND x11 ) ) OR ( ( NOT x2 AND x3 ) AND x15 ) ) OR x2 )
x11 = ( ( ( x2 AND x3 ) AND x15 ) AND x10 )
x12 = x13
x13 = ( ( ( ( ( NOT x6 AND NOT x4 ) AND NOT x15 ) AND x5 ) OR ( ( NOT x6 AND x4 ) AND x5 ) ) OR ( ( x6 AND x4 ) AND x5 ) )
x14 = NOT x17
x15 = x18
x16 = ( NOT x6 AND NOT x1 )
x17 = ( ( ( ( NOT x4 AND NOT x1 ) AND x2 ) OR ( NOT x4 AND x1 ) ) OR ( x4 AND x2 ) )
x18 = ( NOT x16 AND NOT x9 ) \\
MAMMALIAN-CELL-CYCLE & 20 & 1 & 19 & x1: v\_Akt1, x2: v\_CDK2, x3: v\_CDK4, x4: v\_CDK6, x5: v\_CycD1, x6: v\_CycE1, x7: v\_EGF, x8: v\_ERa, x9: v\_ErbB1, x10: v\_ErbB1\_2, x11: v\_ErbB1\_3, x12: v\_ErbB2, x13: v\_ErbB2\_3, x14: v\_ErbB3, x15: v\_IGF1R, x16: v\_MEK1, x17: v\_cMYC, x18: v\_p21, x19: v\_p27, x20: v\_pRB & x1 = ( ( ( ( x13 OR x15 ) OR x10 ) OR x11 ) OR x9 )
x2 = ( x6 AND NOT ( x18 OR x19 ) )
x3 = ( x5 AND NOT ( x18 OR x19 ) )
x4 = x5
x5 = ( ( x1 AND ( x17 AND x8 ) ) OR ( x16 AND ( x8 AND x17 ) ) )
x6 = x17
x8 = ( x1 OR x16 )
x9 = x7
x10 = ( x9 AND x12 )
x11 = ( x9 AND x14 )
x12 = x7
x13 = ( x12 AND x14 )
x14 = x7
x15 = ( ( x8 AND NOT x13 ) OR ( x1 AND NOT x13 ) )
x16 = ( ( ( ( x13 OR x10 ) OR x15 ) OR x11 ) OR x9 )
x17 = ( ( x16 OR x1 ) OR x8 )
x18 = ( x8 AND NOT ( ( x3 OR x1 ) OR x17 ) )
x19 = ( x8 AND NOT ( ( ( x17 OR x3 ) OR x1 ) OR x2 ) )
x20 = ( ( x3 AND x4 ) OR ( x2 AND ( x4 AND x3 ) ) ) \\
CARDIAC-DEVELOPMENT & 15 & 2 & 13 & x1: v\_Bmp2, x2: v\_Dkk1, x3: v\_Fgf8, x4: v\_Foxc1\_2, x5: v\_GATAs, x6: v\_Isl1, x7: v\_Mesp1, x8: v\_Nkx2\_5, x9: v\_Tbx1, x10: v\_Tbx5, x11: v\_canWnt, x12: v\_exogen\_BMP2\_I, x13: v\_exogen\_BMP2\_II, x14: v\_exogen\_CanWnt\_I, x15: v\_exogen\_canWnt\_II & x1 = ( x13 AND NOT x11 )
x2 = ( x7 OR ( x11 AND NOT x13 ) )
x3 = ( ( x9 AND NOT x7 ) OR ( x4 AND NOT x7 ) )
x4 = ( x11 AND x15 )
x5 = ( ( x8 OR x10 ) OR x7 )
x6 = ( ( ( x7 OR x9 ) OR x3 ) OR ( x11 AND x15 ) )
x7 = ( x11 AND NOT x13 )
x8 = ( ( ( ( x10 OR x9 ) OR ( x7 AND x2 ) ) OR ( x1 AND x5 ) ) OR ( x6 AND x5 ) )
x9 = x4
x10 = ( ( ( x10 AND NOT ( ( x11 OR ( x2 AND ( NOT x10 AND NOT x7 ) ) ) OR x9 ) ) OR ( x8 AND NOT ( ( x11 OR ( x2 AND ( NOT x10 AND NOT x7 ) ) ) OR x9 ) ) ) OR ( x7 AND NOT ( ( x11 OR ( x2 AND ( NOT x10 AND NOT x7 ) ) ) OR x9 ) ) )
x11 = x15
x13 = x12
x15 = x14 \\
METABOLIC-INTERACTIONS-IN-GUT-MICROBIOME & 12 & 4 & 8 & x1: v\_Akkermansia\_, x2: v\_Barnesiella, x3: v\_Blautia, x4: v\_Clindamycin\_, x5: v\_Clostridium\_difficile, x6: v\_Coprobacillus, x7: v\_Enterobacteriaceae, x8: v\_Enterococcus, x9: v\_Lachnospiraceae, x10: v\_Lachnospiraceae\_other\_, x11: v\_Mollicutes, x12: v\_Other & x1 = x6
x2 = ( ( ( x10 AND NOT x4 ) OR ( x12 AND NOT x4 ) ) OR ( x9 AND NOT x4 ) )
x3 = ( ( ( ( x6 AND NOT x3 ) OR x8 ) OR ( x3 AND NOT x6 ) ) OR x3 )
x5 = ( x5 AND NOT x2 )
x8 = ( ( ( ( x7 OR x11 ) OR x3 ) OR x5 ) OR NOT ( ( ( ( x7 OR x5 ) OR x6 ) OR x3 ) OR x11 ) )
x9 = ( ( ( x9 AND NOT x4 ) OR ( x10 AND NOT x4 ) ) OR ( x12 AND NOT x4 ) )
x10 = ( ( ( x9 AND NOT x4 ) OR ( x12 AND NOT x4 ) ) OR ( x10 AND NOT x4 ) )
x12 = ( ( ( x12 AND NOT x4 ) OR ( x10 AND NOT x4 ) ) OR ( x9 AND NOT x4 ) ) \\
MORPHOGENETIC-CHECKPOINT & 12 & 1 & 11 & x1: v\_BUD, x2: v\_Clb2\_b1, x3: v\_Clb2\_b2, x4: v\_Hsl1, x5: v\_MASS\_b1, x6: v\_MASS\_b2, x7: v\_Mih1\_b1, x8: v\_Mih1\_b2, x9: v\_Mpk1, x10: v\_SBF, x11: v\_Swe1\_b1, x12: v\_Swe1\_b2 & x1 = x5
x2 = ( ( ( NOT x2 AND x5 ) OR ( ( x2 AND NOT x3 ) AND x5 ) ) OR ( x2 AND x3 ) )
x3 = ( ( ( ( ( ( ( NOT x11 AND x2 ) AND x5 ) OR ( ( ( ( ( x11 AND NOT x12 ) AND NOT x7 ) AND x2 ) AND x5 ) AND x6 ) ) OR ( ( ( ( ( ( x11 AND NOT x12 ) AND x7 ) AND NOT x8 ) AND x2 ) AND x5 ) AND x6 ) ) OR ( ( ( ( ( x11 AND NOT x12 ) AND x7 ) AND x8 ) AND x2 ) AND x5 ) ) OR ( ( ( ( ( ( x11 AND x12 ) AND x7 ) AND NOT x8 ) AND x2 ) AND x5 ) AND x6 ) ) OR ( ( ( ( ( x11 AND x12 ) AND x7 ) AND x8 ) AND x2 ) AND x5 ) )
x4 = x1
x6 = ( x5 AND x6 )
x7 = ( ( ( ( ( ( NOT x7 AND NOT x2 ) AND NOT x9 ) OR ( NOT x7 AND x2 ) ) OR ( ( ( x7 AND NOT x8 ) AND NOT x2 ) AND NOT x9 ) ) OR ( ( x7 AND NOT x8 ) AND x2 ) ) OR ( x7 AND x8 ) )
x8 = ( ( x7 AND x2 ) AND NOT x9 )
x9 = NOT x1
x10 = ( ( NOT x2 AND x5 ) OR ( ( x2 AND NOT x3 ) AND x5 ) )
x11 = ( ( ( ( ( ( ( ( ( NOT x10 AND x11 ) AND x12 ) OR ( ( x10 AND NOT x11 ) AND NOT x2 ) ) OR ( ( ( x10 AND NOT x11 ) AND x2 ) AND NOT x3 ) ) OR ( ( ( ( x10 AND NOT x11 ) AND x2 ) AND x3 ) AND NOT x4 ) ) OR ( ( ( x10 AND x11 ) AND NOT x12 ) AND NOT x2 ) ) OR ( ( ( ( x10 AND x11 ) AND NOT x12 ) AND x2 ) AND NOT x3 ) ) OR ( ( ( ( ( x10 AND x11 ) AND NOT x12 ) AND x2 ) AND x3 ) AND NOT x4 ) ) OR ( ( x10 AND x11 ) AND x12 ) )
x12 = ( ( ( ( x10 AND x11 ) AND NOT x2 ) AND NOT x4 ) OR ( ( ( ( x10 AND x11 ) AND x2 ) AND NOT x3 ) AND NOT x4 ) ) \\
CHICKEN-SEX-DETERMINATION & 15 & 3 & 12 & x1: v\_AMH, x2: v\_AROMA, x3: v\_B\_CATENIN, x4: v\_DMRT1\_b1, x5: v\_DMRT1\_b2, x6: v\_ESTRO, x7: v\_FGF9, x8: v\_FOXL2, x9: v\_HEMGN, x10: v\_SF1, x11: v\_SOX9, x12: v\_W, x13: v\_WNT4, x14: v\_Z1, x15: v\_Z2 & x1 = ( ( ( NOT x11 AND NOT x6 ) AND x10 ) OR ( x11 AND NOT x6 ) )
x2 = ( ( NOT x8 AND x10 ) OR x8 )
x3 = ( NOT x11 AND x13 )
x4 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x14 AND NOT x4 ) AND NOT x9 ) AND x11 ) AND NOT x8 ) OR ( ( ( NOT x14 AND NOT x4 ) AND x9 ) AND NOT x8 ) ) OR ( ( ( ( ( NOT x14 AND x4 ) AND NOT x5 ) AND NOT x9 ) AND x11 ) AND NOT x8 ) ) OR ( ( ( ( NOT x14 AND x4 ) AND NOT x5 ) AND x9 ) AND NOT x8 ) ) OR ( ( NOT x14 AND x4 ) AND x5 ) ) OR ( ( ( ( ( x14 AND NOT x15 ) AND NOT x4 ) AND NOT x9 ) AND x11 ) AND NOT x8 ) ) OR ( ( ( ( x14 AND NOT x15 ) AND NOT x4 ) AND x9 ) AND NOT x8 ) ) OR ( ( ( ( ( ( x14 AND NOT x15 ) AND x4 ) AND NOT x5 ) AND NOT x9 ) AND x11 ) AND NOT x8 ) ) OR ( ( ( ( ( x14 AND NOT x15 ) AND x4 ) AND NOT x5 ) AND x9 ) AND NOT x8 ) ) OR ( ( ( x14 AND NOT x15 ) AND x4 ) AND x5 ) ) OR ( ( ( ( x14 AND x15 ) AND NOT x12 ) AND NOT x4 ) AND NOT x8 ) ) OR ( ( ( ( ( x14 AND x15 ) AND NOT x12 ) AND x4 ) AND NOT x5 ) AND NOT x8 ) ) OR ( ( ( ( x14 AND x15 ) AND NOT x12 ) AND x4 ) AND x5 ) ) OR ( ( ( ( ( ( x14 AND x15 ) AND x12 ) AND NOT x4 ) AND NOT x9 ) AND x11 ) AND NOT x8 ) ) OR ( ( ( ( ( x14 AND x15 ) AND x12 ) AND NOT x4 ) AND x9 ) AND NOT x8 ) ) OR ( ( ( ( ( ( ( x14 AND x15 ) AND x12 ) AND x4 ) AND NOT x5 ) AND NOT x9 ) AND x11 ) AND NOT x8 ) ) OR ( ( ( ( ( ( x14 AND x15 ) AND x12 ) AND x4 ) AND NOT x5 ) AND x9 ) AND NOT x8 ) ) OR ( ( ( ( x14 AND x15 ) AND x12 ) AND x4 ) AND x5 ) )
x5 = ( ( ( ( x4 AND NOT x9 ) AND x11 ) AND NOT x8 ) OR ( ( x4 AND x9 ) AND NOT x8 ) )
x6 = x2
x7 = x11
x8 = ( ( ( ( ( NOT x4 AND NOT x6 ) AND NOT x1 ) OR ( NOT x4 AND x6 ) ) OR ( ( ( x4 AND NOT x5 ) AND NOT x6 ) AND NOT x1 ) ) OR ( ( x4 AND NOT x5 ) AND x6 ) )
x9 = ( x4 AND NOT x11 )
x10 = x6
x11 = ( ( ( ( ( NOT x4 AND x11 ) AND NOT x8 ) AND NOT x3 ) OR ( ( ( ( x4 AND NOT x5 ) AND x11 ) AND NOT x8 ) AND NOT x3 ) ) OR ( ( x4 AND x5 ) AND NOT x8 ) )
x13 = NOT x7 \\
EGGSHELL-PATTERNING-PHENOMOENOLOGICAL & 8 & 4 & 4 & x1: v\_BMP, x2: v\_EGF\_b1, x3: v\_EGF\_b2, x4: v\_Floor, x5: v\_Operculum, x6: v\_Roof, x7: v\_Roof\_adj, x8: v\_anterior & x3 = ( x2 AND x3 )
x4 = ( ( ( ( ( x2 AND NOT x3 ) AND x1 ) AND x7 ) AND x8 ) OR ( ( ( x2 AND x3 ) AND x7 ) AND x8 ) )
x5 = ( ( ( ( ( x2 AND NOT x3 ) AND x1 ) AND NOT x7 ) AND x8 ) OR ( ( ( x2 AND x3 ) AND NOT x7 ) AND x8 ) )
x6 = ( ( ( x2 AND NOT x3 ) AND NOT x1 ) AND x8 ) \\
OXIDATIVE-STRESS-PATHWAY & 19 & 1 & 18 & x1: v\_ARE, x2: v\_ATM, x3: v\_Akt, x4: v\_Bach1, x5: v\_Bad, x6: v\_Bcl2, x7: v\_GSK3b, x8: v\_Keap1, x9: v\_Mdm2, x10: v\_Nrf2, x11: v\_PI3K, x12: v\_PIP2, x13: v\_PIP3, x14: v\_PKC, x15: v\_PTEN, x16: v\_ROS, x17: v\_Ras, x18: v\_Stress, x19: v\_p53 & x1 = ( x10 AND NOT ( ( x7 OR x4 ) OR x1 ) )
x2 = x16
x3 = x13
x4 = NOT x16
x5 = NOT x3
x6 = NOT ( x19 OR x5 )
x7 = NOT x3
x8 = ( ( x10 AND NOT x4 ) OR ( x8 AND NOT x4 ) )
x9 = ( ( x19 AND NOT x2 ) OR ( x3 AND NOT x2 ) )
x10 = ( ( x14 OR x3 ) OR NOT ( ( x3 OR x8 ) OR x14 ) )
x11 = x17
x12 = x11
x13 = ( x12 AND NOT x15 )
x14 = ( x16 AND ( NOT x1 OR NOT x1 ) )
x15 = NOT x16
x16 = ( x18 AND NOT x1 )
x17 = x16
x19 = ( x2 AND NOT x9 ) \\
CORTICAL-AREA-DEVELOPMENT & 5 & 0 & 5 & x1: v\_Coup\_fti, x2: v\_Emx2, x3: v\_Fgf8, x4: v\_Pax6, x5: v\_Sp8 & x1 = ( NOT ( x3 OR x5 ) OR NOT ( x5 OR x3 ) )
x2 = ( x1 AND NOT ( ( x3 OR x5 ) OR x4 ) )
x3 = ( ( x3 AND x5 ) AND NOT x2 )
x4 = ( x5 AND NOT ( x2 OR x1 ) )
x5 = ( x3 AND NOT x2 ) \\
BUDDING-YEAST-EXIT-MODULE & 16 & 5 & 11 & x1: v\_Bub2\_Bfa1, x2: v\_Cdc14, x3: v\_Cdc15, x4: v\_Cdc20, x5: v\_Cdc5Polo, x6: v\_Cdh1, x7: v\_Clb2\_b1, x8: v\_Clb2\_b2, x9: v\_Net1\_b1, x10: v\_Net1\_b2, x11: v\_PP2ACdc55\_b1, x12: v\_PP2ACdc55\_b2, x13: v\_SecurinPds1, x14: v\_SeparaseEsp1\_b1, x15: v\_SeparaseEsp1\_b2, x16: v\_Tem1 & x1 = ( ( ( NOT x11 AND NOT x5 ) OR ( ( x11 AND NOT x12 ) AND NOT x5 ) ) OR ( x11 AND x12 ) )
x3 = ( ( ( NOT x7 OR ( x7 AND NOT x8 ) ) OR ( ( ( x7 AND x8 ) AND NOT x9 ) AND x2 ) ) OR ( ( ( ( x7 AND x8 ) AND x9 ) AND NOT x10 ) AND x2 ) )
x4 = NOT x6
x5 = ( x7 AND NOT x6 )
x6 = ( ( ( ( ( ( NOT x7 AND NOT x9 ) AND NOT x2 ) AND x6 ) OR ( ( NOT x7 AND NOT x9 ) AND x2 ) ) OR ( ( NOT x7 AND x9 ) AND x6 ) ) OR ( ( ( x7 AND NOT x8 ) AND NOT x9 ) AND x2 ) )
x7 = ( ( ( NOT x7 AND NOT x6 ) OR ( ( x7 AND NOT x8 ) AND NOT x6 ) ) OR ( x7 AND x8 ) )
x8 = ( ( x7 AND NOT x4 ) AND NOT x6 )
x9 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x7 AND NOT x11 ) AND NOT x1 ) AND NOT x16 ) AND NOT x9 ) AND x2 ) OR ( ( ( ( ( ( NOT x7 AND NOT x11 ) AND NOT x1 ) AND NOT x16 ) AND x9 ) AND NOT x10 ) AND x2 ) ) OR ( ( ( ( ( NOT x7 AND NOT x11 ) AND NOT x1 ) AND NOT x16 ) AND x9 ) AND x10 ) ) OR ( ( ( ( ( ( NOT x7 AND NOT x11 ) AND NOT x1 ) AND x16 ) AND NOT x3 ) AND NOT x9 ) AND x2 ) ) OR ( ( ( ( ( ( ( NOT x7 AND NOT x11 ) AND NOT x1 ) AND x16 ) AND NOT x3 ) AND x9 ) AND NOT x10 ) AND x2 ) ) OR ( ( ( ( ( ( NOT x7 AND NOT x11 ) AND NOT x1 ) AND x16 ) AND NOT x3 ) AND x9 ) AND x10 ) ) OR ( ( ( ( ( ( NOT x7 AND NOT x11 ) AND NOT x1 ) AND x16 ) AND x3 ) AND x9 ) AND x10 ) ) OR ( ( ( ( NOT x7 AND NOT x11 ) AND x1 ) AND NOT x9 ) AND x2 ) ) OR ( ( ( ( ( NOT x7 AND NOT x11 ) AND x1 ) AND x9 ) AND NOT x10 ) AND x2 ) ) OR ( ( ( ( NOT x7 AND NOT x11 ) AND x1 ) AND x9 ) AND x10 ) ) OR ( ( ( NOT x7 AND x11 ) AND NOT x1 ) AND NOT x16 ) ) OR ( ( ( ( NOT x7 AND x11 ) AND NOT x1 ) AND x16 ) AND NOT x3 ) ) OR ( ( ( ( ( ( NOT x7 AND x11 ) AND NOT x1 ) AND x16 ) AND x3 ) AND x9 ) AND x10 ) ) OR ( ( NOT x7 AND x11 ) AND x1 ) ) OR ( ( ( ( x7 AND NOT x8 ) AND NOT x11 ) AND x9 ) AND x10 ) ) OR ( ( ( ( x7 AND NOT x8 ) AND x11 ) AND NOT x1 ) AND NOT x16 ) ) OR ( ( ( ( ( x7 AND NOT x8 ) AND x11 ) AND NOT x1 ) AND x16 ) AND NOT x3 ) ) OR ( ( ( ( ( ( ( x7 AND NOT x8 ) AND x11 ) AND NOT x1 ) AND x16 ) AND x3 ) AND x9 ) AND x10 ) ) OR ( ( ( x7 AND NOT x8 ) AND x11 ) AND x1 ) ) OR ( ( ( ( x7 AND x8 ) AND NOT x11 ) AND x9 ) AND x10 ) ) OR ( ( ( ( ( x7 AND x8 ) AND x11 ) AND NOT x12 ) AND x9 ) AND x10 ) ) OR ( ( ( ( ( x7 AND x8 ) AND x11 ) AND x12 ) AND NOT x1 ) AND NOT x16 ) ) OR ( ( ( ( ( ( x7 AND x8 ) AND x11 ) AND x12 ) AND NOT x1 ) AND x16 ) AND NOT x3 ) ) OR ( ( ( ( ( ( ( ( x7 AND x8 ) AND x11 ) AND x12 ) AND NOT x1 ) AND x16 ) AND x3 ) AND x9 ) AND x10 ) ) OR ( ( ( ( x7 AND x8 ) AND x11 ) AND x12 ) AND x1 ) )
x10 = ( ( ( ( ( ( ( ( ( NOT x7 AND x11 ) AND NOT x1 ) AND NOT x16 ) AND x9 ) OR ( ( ( ( ( NOT x7 AND x11 ) AND NOT x1 ) AND x16 ) AND NOT x3 ) AND x9 ) ) OR ( ( ( NOT x7 AND x11 ) AND x1 ) AND x9 ) ) OR ( ( ( ( ( x7 AND x11 ) AND x12 ) AND NOT x1 ) AND NOT x16 ) AND x9 ) ) OR ( ( ( ( ( ( x7 AND x11 ) AND x12 ) AND NOT x1 ) AND x16 ) AND NOT x3 ) AND x9 ) ) OR ( ( ( ( x7 AND x11 ) AND x12 ) AND x1 ) AND x9 ) )
x12 = ( ( ( ( NOT x13 AND NOT x14 ) AND x11 ) OR ( ( x13 AND NOT x14 ) AND x11 ) ) OR ( ( ( x13 AND x14 ) AND NOT x15 ) AND x11 ) )
x13 = NOT x4 \\
ASYMMETRIC-CELL-DIVISION-A & 5 & 0 & 5 & x1: v\_CcrM, x2: v\_CtrA, x3: v\_DnaA, x4: v\_GcrA, x5: v\_SciP & x1 = ( ( x2 AND NOT x1 ) AND NOT x5 )
x2 = ( ( ( ( NOT x2 AND x4 ) AND NOT x1 ) AND NOT x5 ) OR ( ( x2 AND NOT x1 ) AND NOT x5 ) )
x3 = ( ( ( x2 AND NOT x4 ) AND NOT x3 ) AND x1 )
x4 = ( NOT x2 AND x3 )
x5 = ( x2 AND NOT x3 ) \\
BODY-SEGMENTATION-IN-DROSOPHILA-2013 & 17 & 3 & 14 & x1: v\_CIA, x2: v\_CIR, x3: v\_CI\_protein, x4: v\_EN\_protein, x5: v\_HH\_protein, x6: v\_PH, x7: v\_PTC\_protein, x8: v\_SLP, x9: v\_SMO, x10: v\_WG\_external, x11: v\_WG\_protein, x12: v\_ci, x13: v\_en, x14: v\_hh, x15: v\_hh\_external, x16: v\_ptc, x17: v\_wg & x1 = ( ( x15 AND x3 ) OR ( x3 AND NOT x7 ) )
x2 = ( ( x3 AND x7 ) AND NOT x15 )
x3 = x12
x4 = x13
x5 = x14
x6 = ( x7 AND x15 )
x7 = ( ( x7 AND NOT x15 ) OR x16 )
x9 = ( x15 OR NOT ( x15 OR x7 ) )
x11 = x17
x12 = NOT x4
x13 = ( x10 AND NOT x8 )
x14 = ( x4 AND NOT x2 )
x16 = ( x1 AND NOT ( x2 OR x4 ) )
x17 = ( ( ( x17 AND ( x8 OR x1 ) ) AND NOT x2 ) OR ( ( x1 AND x8 ) AND NOT x2 ) ) \\
DROSOPHILA-GAP-D & 7 & 2 & 5 & x1: v\_Gt, x2: v\_Hb\_b1, x3: v\_Hb\_b2, x4: v\_Hb\_b3, x5: v\_Kni, x6: v\_Kr\_b1, x7: v\_Kr\_b2 & x1 = ( NOT x2 AND NOT x6 )
x2 = ( x2 AND x3 )
x3 = ( ( x2 AND x3 ) AND x4 )
x5 = ( ( NOT x1 AND NOT x2 ) OR ( ( NOT x1 AND x2 ) AND NOT x3 ) )
x6 = ( x6 AND x7 ) \\
DROSOPHILA-DPP-PATHWAY & 18 & 8 & 10 & x1: v\_Brk, x2: v\_Dad, x3: v\_Dpp\_b1, x4: v\_Dpp\_b2, x5: v\_Gbb, x6: v\_MadMed\_b1, x7: v\_MadMed\_b2, x8: v\_Nej, x9: v\_Punt, x10: v\_Sax, x11: v\_Scw, x12: v\_Shn, x13: v\_Sog, x14: v\_Targets, x15: v\_Tkv\_b1, x16: v\_Tkv\_b2, x17: v\_Tld, x18: v\_Tsg & x1 = ( NOT x12 AND NOT x6 )
x2 = ( ( NOT x1 AND x6 ) AND x7 )
x4 = ( x3 AND x4 )
x6 = ( ( ( ( ( ( ( ( NOT x15 AND NOT x10 ) AND x6 ) AND x7 ) OR ( ( NOT x15 AND x10 ) AND NOT x2 ) ) OR ( ( ( ( NOT x15 AND x10 ) AND x2 ) AND x6 ) AND x7 ) ) OR ( ( x15 AND NOT x16 ) AND NOT x2 ) ) OR ( ( ( ( x15 AND NOT x16 ) AND x2 ) AND x6 ) AND x7 ) ) OR ( x15 AND x16 ) )
x7 = ( ( ( x15 AND x16 ) AND NOT x2 ) AND x6 )
x10 = ( ( ( ( ( ( NOT x11 AND NOT x5 ) AND NOT x13 ) AND x3 ) AND x9 ) OR ( ( ( NOT x11 AND x5 ) AND NOT x13 ) AND x9 ) ) OR ( ( x11 AND NOT x13 ) AND x9 ) )
x13 = NOT x17
x14 = ( ( NOT x1 AND x6 ) AND x8 )
x15 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x11 AND NOT x5 ) AND NOT x13 ) AND NOT x3 ) AND x15 ) AND x16 ) OR ( ( ( ( ( ( NOT x11 AND NOT x5 ) AND NOT x13 ) AND x3 ) AND NOT x18 ) AND NOT x15 ) AND x9 ) ) OR ( ( ( ( ( ( ( NOT x11 AND NOT x5 ) AND NOT x13 ) AND x3 ) AND NOT x18 ) AND x15 ) AND NOT x16 ) AND x9 ) ) OR ( ( ( ( ( ( NOT x11 AND NOT x5 ) AND NOT x13 ) AND x3 ) AND NOT x18 ) AND x15 ) AND x16 ) ) OR ( ( ( ( ( ( NOT x11 AND NOT x5 ) AND NOT x13 ) AND x3 ) AND x18 ) AND x15 ) AND x16 ) ) OR ( ( ( ( NOT x11 AND NOT x5 ) AND x13 ) AND x15 ) AND x16 ) ) OR ( ( ( ( ( NOT x11 AND x5 ) AND NOT x13 ) AND NOT x18 ) AND NOT x15 ) AND x9 ) ) OR ( ( ( ( ( ( NOT x11 AND x5 ) AND NOT x13 ) AND NOT x18 ) AND x15 ) AND NOT x16 ) AND x9 ) ) OR ( ( ( ( ( NOT x11 AND x5 ) AND NOT x13 ) AND NOT x18 ) AND x15 ) AND x16 ) ) OR ( ( ( ( ( NOT x11 AND x5 ) AND NOT x13 ) AND x18 ) AND x15 ) AND x16 ) ) OR ( ( ( ( NOT x11 AND x5 ) AND x13 ) AND x15 ) AND x16 ) ) OR ( ( ( ( x11 AND NOT x13 ) AND NOT x18 ) AND NOT x15 ) AND x9 ) ) OR ( ( ( ( ( x11 AND NOT x13 ) AND NOT x18 ) AND x15 ) AND NOT x16 ) AND x9 ) ) OR ( ( ( ( x11 AND NOT x13 ) AND NOT x18 ) AND x15 ) AND x16 ) ) OR ( ( ( ( x11 AND NOT x13 ) AND x18 ) AND x15 ) AND x16 ) ) OR ( ( ( x11 AND x13 ) AND x15 ) AND x16 ) )
x16 = ( ( ( ( ( NOT x13 AND x3 ) AND x4 ) AND NOT x18 ) AND x15 ) AND x9 ) \\
DROSOPHILA-GAP-B & 7 & 3 & 4 & x1: v\_Gt, x2: v\_Hb\_b1, x3: v\_Hb\_b2, x4: v\_Hb\_b3, x5: v\_Kni, x6: v\_Kr\_b1, x7: v\_Kr\_b2 & x1 = NOT x6
x3 = x2
x6 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x1 AND NOT x2 ) AND x6 ) AND x7 ) OR ( ( NOT x1 AND x2 ) AND NOT x3 ) ) OR ( ( ( NOT x1 AND x2 ) AND x3 ) AND NOT x4 ) ) OR ( ( ( ( ( NOT x1 AND x2 ) AND x3 ) AND x4 ) AND x6 ) AND x7 ) ) OR ( ( ( x1 AND NOT x2 ) AND x6 ) AND x7 ) ) OR ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND NOT x6 ) AND NOT x5 ) ) OR ( ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND x6 ) AND NOT x7 ) AND NOT x5 ) ) OR ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND x6 ) AND x7 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND NOT x6 ) AND NOT x5 ) ) OR ( ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND NOT x7 ) AND NOT x5 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND x7 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND x4 ) AND x6 ) AND x7 ) )
x7 = ( ( ( ( ( NOT x1 AND x2 ) AND NOT x3 ) AND x6 ) AND NOT x5 ) OR ( ( ( ( ( NOT x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND NOT x5 ) ) \\
DROSOPHILA-CELL-CYCLE & 14 & 3 & 11 & x1: v\_Ago, x2: v\_CycA, x3: v\_CycB, x4: v\_CycD, x5: v\_CycE, x6: v\_Dap, x7: v\_E2F, x8: v\_Fzr, x9: v\_Fzy, x10: v\_Notch, x11: v\_Rb, x12: v\_Rux, x13: v\_Stg, x14: v\_Wee1 & x2 = ( ( ( NOT x11 AND x7 ) AND NOT x9 ) AND NOT x8 )
x3 = ( ( ( NOT x9 AND NOT x8 ) AND NOT x14 ) OR ( ( ( NOT x9 AND NOT x8 ) AND x14 ) AND x13 ) )
x5 = ( ( ( NOT x11 AND x7 ) AND NOT x6 ) OR ( ( ( NOT x11 AND x7 ) AND x6 ) AND NOT x1 ) )
x6 = ( ( NOT x5 AND NOT x10 ) OR x5 )
x7 = ( ( ( ( ( NOT x11 AND NOT x2 ) AND NOT x12 ) AND NOT x3 ) OR ( ( NOT x11 AND NOT x2 ) AND x12 ) ) OR ( ( NOT x11 AND x2 ) AND x12 ) )
x8 = ( ( ( ( ( ( ( ( NOT x5 AND NOT x2 ) AND NOT x12 ) AND NOT x3 ) OR ( ( NOT x5 AND NOT x2 ) AND x12 ) ) OR ( ( NOT x5 AND x2 ) AND x12 ) ) OR ( ( ( ( x5 AND NOT x2 ) AND NOT x12 ) AND NOT x3 ) AND x10 ) ) OR ( ( ( x5 AND NOT x2 ) AND x12 ) AND x10 ) ) OR ( ( ( x5 AND x2 ) AND x12 ) AND x10 ) )
x9 = ( NOT x12 AND x3 )
x11 = ( ( ( ( ( ( NOT x4 AND NOT x5 ) AND NOT x2 ) AND NOT x12 ) AND NOT x3 ) OR ( ( ( NOT x4 AND NOT x5 ) AND NOT x2 ) AND x12 ) ) OR ( ( ( NOT x4 AND NOT x5 ) AND x2 ) AND x12 ) )
x12 = ( ( ( ( ( ( ( ( NOT x4 AND NOT x2 ) AND NOT x12 ) AND NOT x3 ) OR ( ( NOT x4 AND NOT x2 ) AND x12 ) ) OR ( ( ( NOT x4 AND x2 ) AND x12 ) AND NOT x3 ) ) OR ( ( ( ( x4 AND NOT x5 ) AND NOT x2 ) AND NOT x12 ) AND NOT x3 ) ) OR ( ( ( x4 AND NOT x5 ) AND NOT x2 ) AND x12 ) ) OR ( ( ( ( x4 AND NOT x5 ) AND x2 ) AND x12 ) AND NOT x3 ) )
x13 = ( ( ( ( ( ( NOT x11 AND NOT x7 ) AND NOT x12 ) AND x3 ) AND NOT x10 ) OR ( ( NOT x11 AND x7 ) AND NOT x10 ) ) OR ( ( ( x11 AND NOT x12 ) AND x3 ) AND NOT x10 ) )
x14 = ( ( NOT x12 AND NOT x3 ) OR x12 ) \\
MAPK-REDUCED-1 & 17 & 4 & 13 & x1: v\_AKT, x2: v\_Apoptosis, x3: v\_DNA\_damage, x4: v\_EGFR, x5: v\_EGFR\_stimulus, x6: v\_ERK, x7: v\_FGFR3, x8: v\_FGFR3\_stimulus, x9: v\_FRS2, x10: v\_Growth\_Arrest, x11: v\_MSK, x12: v\_PI3K, x13: v\_PTEN, x14: v\_Proliferation, x15: v\_TGFBR\_stimulus, x16: v\_p14, x17: v\_p53 & x1 = ( x12 AND NOT x13 )
x2 = ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND NOT x1 ) AND NOT x11 ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) AND NOT x1 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND x7 ) AND NOT x1 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND x4 ) AND NOT x1 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND x17 ) AND NOT x1 ) ) OR ( ( ( x15 AND NOT x6 ) AND x17 ) AND NOT x1 ) )
x4 = ( ( ( ( ( ( NOT x5 AND NOT x15 ) AND x6 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) OR ( ( ( ( x5 AND NOT x15 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) )
x6 = ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) AND x11 ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND x11 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND x4 ) AND x11 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND x11 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND x4 ) AND x11 ) )
x7 = ( ( ( ( x8 AND NOT x15 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 )
x9 = ( ( ( ( NOT x15 AND NOT x6 ) AND NOT x4 ) AND x7 ) AND NOT x9 )
x10 = ( x17 AND NOT x1 )
x11 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) AND NOT x11 ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND NOT x11 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND x4 ) AND NOT x11 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND NOT x11 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND x7 ) ) OR ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND x4 ) ) OR ( ( NOT x15 AND NOT x3 ) AND x6 ) ) OR ( ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND NOT x11 ) ) OR ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) ) OR ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND x4 ) ) OR ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND x17 ) ) OR ( ( NOT x15 AND x3 ) AND x6 ) ) OR x15 )
x12 = ( ( ( ( ( ( NOT x15 AND NOT x4 ) AND NOT x9 ) AND x12 ) OR ( ( NOT x15 AND NOT x4 ) AND x9 ) ) OR ( NOT x15 AND x4 ) ) OR x15 )
x13 = x17
x14 = ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND x12 ) AND x1 ) AND x11 ) OR ( ( ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x12 ) AND x1 ) AND x11 ) ) OR ( ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND x12 ) AND x11 ) ) OR ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND x4 ) AND x12 ) AND x11 ) ) OR ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND x17 ) AND x12 ) AND x1 ) AND x11 ) ) OR ( ( ( ( x15 AND x6 ) AND NOT x17 ) AND x12 ) AND x11 ) ) OR ( ( ( ( ( x15 AND x6 ) AND x17 ) AND x12 ) AND x1 ) AND x11 ) )
x16 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND x1 ) AND x11 ) OR ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND x1 ) AND x11 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) AND x11 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND x7 ) AND x11 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND x4 ) AND x11 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND x1 ) AND x11 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND x1 ) AND x11 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND x17 ) AND NOT x4 ) AND x7 ) AND x11 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND x17 ) AND x4 ) AND x11 ) ) OR ( ( ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND x1 ) AND x11 ) ) OR ( ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) AND x11 ) ) OR ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND x11 ) ) OR ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND x4 ) AND x11 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND x17 ) AND x11 ) ) OR ( ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x1 ) AND x11 ) ) OR ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND x11 ) ) OR ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND x4 ) AND x11 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND x17 ) AND x11 ) ) OR ( x15 AND x11 ) )
x17 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) AND NOT x1 ) AND NOT x11 ) OR ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) AND x1 ) AND NOT x11 ) AND x16 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND NOT x1 ) AND NOT x11 ) ) OR ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND x1 ) AND NOT x11 ) AND x16 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND x4 ) AND NOT x1 ) AND NOT x11 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND NOT x17 ) AND x4 ) AND x1 ) AND NOT x11 ) AND x16 ) ) OR ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND NOT x11 ) AND x16 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) AND x16 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND NOT x4 ) AND x7 ) AND x16 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND NOT x6 ) AND x17 ) AND x4 ) AND x16 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND NOT x1 ) AND NOT x11 ) ) OR ( ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) AND x1 ) AND NOT x11 ) AND x16 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND x4 ) AND NOT x1 ) AND NOT x11 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND NOT x17 ) AND x4 ) AND x1 ) AND NOT x11 ) AND x16 ) ) OR ( ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x11 ) AND x16 ) ) OR ( ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND x17 ) AND NOT x4 ) AND x7 ) AND x16 ) ) OR ( ( ( ( ( NOT x15 AND NOT x3 ) AND x6 ) AND x17 ) AND x4 ) AND x16 ) ) OR ( ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND NOT x1 ) ) OR ( ( ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND x1 ) AND NOT x11 ) ) OR ( ( ( ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x9 ) AND x1 ) AND x11 ) AND x16 ) ) OR ( ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x9 ) ) OR ( ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND NOT x17 ) AND x4 ) ) OR ( ( ( NOT x15 AND x3 ) AND NOT x6 ) AND x17 ) ) OR ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND NOT x1 ) ) OR ( ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x1 ) AND NOT x11 ) ) OR ( ( ( ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND NOT x7 ) AND x1 ) AND x11 ) AND x16 ) ) OR ( ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND NOT x4 ) AND x7 ) ) OR ( ( ( ( NOT x15 AND x3 ) AND x6 ) AND NOT x17 ) AND x4 ) ) OR ( ( ( NOT x15 AND x3 ) AND x6 ) AND x17 ) ) OR ( ( ( x15 AND NOT x3 ) AND NOT x17 ) AND NOT x1 ) ) OR ( ( ( ( x15 AND NOT x3 ) AND NOT x17 ) AND x1 ) AND x16 ) ) OR ( ( ( x15 AND NOT x3 ) AND x17 ) AND x16 ) ) OR ( x15 AND x3 ) ) \\
BUDDING-YEAST-CELL-CYCLE-2009 & 18 & 0 & 18 & x1: v\_B, x2: v\_CD, x3: v\_CKI, x4: v\_Cdc14, x5: v\_Cdc20, x6: v\_Cdh1, x7: v\_Clb2, x8: v\_Clb5, x9: v\_Cln2, x10: v\_Cln3, x11: v\_FEAR, x12: v\_M, x13: v\_MEN, x14: v\_S, x15: v\_SFF, x16: v\_SMBF, x17: v\_Swi5, x18: v\_Yhp1 & x1 = ( ( ( x9 AND NOT x2 ) OR ( x1 AND NOT x2 ) ) OR ( x8 AND NOT x2 ) )
x2 = ( ( x12 AND ( x4 AND x11 ) ) AND NOT x2 )
x3 = ( ( ( x17 AND NOT ( ( x7 OR x9 ) OR x8 ) ) OR ( x3 AND NOT ( ( x7 OR x9 ) OR x8 ) ) ) OR ( x4 AND x17 ) )
x4 = ( x11 AND x13 )
x5 = ( x12 AND ( x15 AND x7 ) )
x6 = ( x4 OR NOT ( ( ( x4 OR x8 ) OR x9 ) OR x7 ) )
x7 = ( ( ( x1 AND ( NOT x5 OR NOT x6 ) ) AND NOT x3 ) OR ( ( x7 AND ( ( NOT x5 OR NOT x6 ) AND x15 ) ) AND NOT x3 ) )
x8 = ( x16 AND ( NOT x5 OR ( NOT x3 AND NOT x5 ) ) )
x9 = x16
x10 = NOT x18
x11 = x5
x12 = ( ( x12 AND NOT x2 ) OR ( ( x14 AND x7 ) AND NOT x2 ) )
x13 = ( x11 AND x7 )
x14 = ( ( ( x8 AND NOT x2 ) OR ( x7 AND NOT x2 ) ) OR ( x14 AND NOT x2 ) )
x15 = ( ( x7 AND x15 ) OR ( ( x1 AND ( NOT x5 OR NOT x6 ) ) AND NOT x3 ) )
x16 = ( ( ( x10 AND NOT x7 ) OR ( x16 AND NOT x7 ) ) OR ( x9 AND NOT x7 ) )
x17 = ( ( x4 AND x15 ) OR ( x15 AND NOT x7 ) )
x18 = x16 \\
REGULATION-OF-L-ARABINOSE-OPERON & 13 & 4 & 9 & x1: v\_A, x2: v\_Ae, x3: v\_Aem, x4: v\_Am, x5: v\_C, x6: v\_E, x7: v\_Ge, x8: v\_L, x9: v\_MS, x10: v\_MT, x11: v\_S\_2\_Ara\_, x12: v\_S\_7\_Ara\_, x13: v\_T & x1 = ( x2 AND x13 )
x4 = ( ( x3 AND x13 ) OR x2 )
x5 = NOT x7
x6 = x9
x8 = ( x11 AND NOT x12 )
x9 = ( x12 AND x5 )
x10 = ( x12 AND x5 )
x12 = ( x11 AND ( x1 OR x4 ) )
x13 = x10 \\
HEPATOCELLULAR-CARCINOMA-REDUCED & 19 & 0 & 19 & x1: v\_AKT, x2: v\_AXIN2, x3: v\_Bcatenin\_memb, x4: v\_Bcatenin\_nuc, x5: v\_Dest\_compl, x6: v\_Ecadherin, x7: v\_GLI, x8: v\_GSK3B, x9: v\_MEK, x10: v\_NOTCH, x11: v\_SMAD, x12: v\_SNAI1, x13: v\_SNAI2, x14: v\_SOS\_GRB2, x15: v\_TGFBR, x16: v\_TWIST1, x17: v\_ZEB1, x18: v\_ZEB2, x19: v\_miR200 & x1 = ( x11 OR ( x14 OR ( NOT x8 OR x4 ) ) )
x2 = ( x2 OR x4 )
x3 = ( x6 AND NOT x4 )
x4 = ( NOT x5 AND ( NOT x3 AND ( x11 OR ( x7 OR NOT x6 ) ) ) )
x5 = ( ( x8 AND ( x2 AND x4 ) ) OR ( x8 AND x5 ) )
x6 = ( x3 AND ( NOT x12 OR ( ( NOT x10 AND NOT x11 ) OR ( NOT x17 OR ( NOT x18 OR ( NOT x16 OR NOT x13 ) ) ) ) ) )
x7 = ( x4 OR ( x11 OR x7 ) )
x8 = ( NOT x7 AND NOT x1 )
x9 = ( x14 OR ( NOT x8 OR ( x4 OR NOT ( NOT x9 OR NOT x12 ) ) ) )
x10 = ( x14 OR ( NOT x8 OR ( x4 OR x11 ) ) )
x11 = ( ( x9 OR x15 ) AND ( x17 OR NOT x18 ) )
x12 = ( x7 OR ( x11 OR ( x4 OR ( x15 OR ( x10 OR ( x9 OR ( x1 OR NOT x8 ) ) ) ) ) ) )
x13 = ( x9 OR ( x4 OR ( x13 OR x16 ) ) )
x14 = ( ( x4 OR x15 ) AND NOT x9 )
x15 = ( x12 OR ( x16 OR x7 ) )
x16 = ( x1 OR ( x4 OR x12 ) )
x17 = ( x12 AND NOT x19 )
x18 = ( x12 AND NOT x19 )
x19 = ( NOT x12 AND ( NOT x17 AND NOT x18 ) ) \\
MAPK-REDUCED-3 & 16 & 4 & 12 & x1: v\_Apoptosis, x2: v\_DNA\_damage, x3: v\_EGFR\_stimulus, x4: v\_ERK, x5: v\_FGFR3\_stimulus, x6: v\_GADD45, x7: v\_GRB2, x8: v\_Growth\_Arrest, x9: v\_JNK, x10: v\_MDM2, x11: v\_PI3K, x12: v\_PLCG, x13: v\_Proliferation, x14: v\_RAS, x15: v\_TGFBR\_stimulus, x16: v\_p38 & x1 = ( ( ( ( ( ( NOT x2 AND NOT x4 ) AND x16 ) AND x9 ) AND NOT x10 ) OR ( ( ( ( x2 AND NOT x4 ) AND NOT x16 ) AND x9 ) AND NOT x10 ) ) OR ( ( ( x2 AND NOT x4 ) AND x16 ) AND x9 ) )
x4 = ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x2 AND NOT x4 ) AND NOT x16 ) AND NOT x9 ) AND NOT x12 ) AND x14 ) OR ( ( ( ( ( NOT x2 AND NOT x4 ) AND NOT x16 ) AND NOT x9 ) AND x12 ) AND NOT x11 ) ) OR ( ( ( ( ( ( NOT x2 AND NOT x4 ) AND NOT x16 ) AND NOT x9 ) AND x12 ) AND x11 ) AND x14 ) ) OR ( ( ( ( NOT x2 AND x4 ) AND NOT x16 ) AND NOT x9 ) AND x14 ) ) OR ( ( ( ( ( x2 AND NOT x4 ) AND NOT x16 ) AND NOT x9 ) AND NOT x12 ) AND x14 ) ) OR ( ( ( ( ( x2 AND NOT x4 ) AND NOT x16 ) AND NOT x9 ) AND x12 ) AND NOT x11 ) ) OR ( ( ( ( ( ( ( x2 AND NOT x4 ) AND NOT x16 ) AND NOT x9 ) AND x12 ) AND x11 ) AND NOT x14 ) AND NOT x10 ) ) OR ( ( ( ( ( ( x2 AND NOT x4 ) AND NOT x16 ) AND NOT x9 ) AND x12 ) AND x11 ) AND x14 ) ) OR ( ( ( ( x2 AND x4 ) AND NOT x16 ) AND NOT x9 ) AND x14 ) )
x6 = ( ( ( ( ( ( NOT x15 AND NOT x2 ) AND x16 ) AND NOT x10 ) OR ( ( ( NOT x15 AND x2 ) AND NOT x16 ) AND NOT x10 ) ) OR ( ( NOT x15 AND x2 ) AND x16 ) ) OR x15 )
x7 = ( ( ( ( ( ( ( ( ( ( NOT x3 AND NOT x5 ) AND NOT x15 ) AND x4 ) AND NOT x7 ) AND NOT x12 ) OR ( ( NOT x3 AND NOT x5 ) AND x15 ) ) OR ( ( ( ( NOT x3 AND x5 ) AND NOT x15 ) AND NOT x7 ) AND NOT x12 ) ) OR ( ( NOT x3 AND x5 ) AND x15 ) ) OR ( ( ( x3 AND NOT x15 ) AND NOT x7 ) AND NOT x12 ) ) OR ( x3 AND x15 ) )
x8 = ( ( ( ( NOT x2 AND x16 ) AND NOT x10 ) OR ( ( x2 AND NOT x16 ) AND NOT x10 ) ) OR ( x2 AND x16 ) )
x9 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x2 ) AND NOT x4 ) AND NOT x16 ) AND NOT x6 ) AND x14 ) OR ( ( ( ( NOT x15 AND NOT x2 ) AND NOT x4 ) AND NOT x16 ) AND x6 ) ) OR ( ( ( ( ( NOT x15 AND NOT x2 ) AND NOT x4 ) AND x16 ) AND x6 ) AND x14 ) ) OR ( ( ( ( NOT x15 AND NOT x2 ) AND x4 ) AND x6 ) AND x14 ) ) OR ( ( ( NOT x15 AND x2 ) AND NOT x4 ) AND NOT x16 ) ) OR ( ( ( ( ( NOT x15 AND x2 ) AND NOT x4 ) AND x16 ) AND NOT x6 ) AND x14 ) ) OR ( ( ( ( NOT x15 AND x2 ) AND NOT x4 ) AND x16 ) AND x6 ) ) OR ( ( ( ( NOT x15 AND x2 ) AND x4 ) AND NOT x6 ) AND x14 ) ) OR ( ( ( NOT x15 AND x2 ) AND x4 ) AND x6 ) ) OR ( ( ( x15 AND NOT x2 ) AND NOT x4 ) AND NOT x16 ) ) OR ( ( ( ( ( x15 AND NOT x2 ) AND NOT x4 ) AND x16 ) AND NOT x6 ) AND x14 ) ) OR ( ( ( ( x15 AND NOT x2 ) AND NOT x4 ) AND x16 ) AND x6 ) ) OR ( ( ( ( x15 AND NOT x2 ) AND x4 ) AND NOT x6 ) AND x14 ) ) OR ( ( ( x15 AND NOT x2 ) AND x4 ) AND x6 ) ) OR ( x15 AND x2 ) )
x10 = ( ( ( ( ( ( NOT x2 AND NOT x4 ) AND NOT x16 ) AND x11 ) OR ( ( ( ( x2 AND NOT x4 ) AND NOT x16 ) AND NOT x11 ) AND NOT x10 ) ) OR ( ( ( x2 AND NOT x4 ) AND NOT x16 ) AND x11 ) ) OR ( ( ( x2 AND x4 ) AND NOT x16 ) AND NOT x10 ) )
x11 = ( ( NOT x7 AND x11 ) OR x7 )
x12 = ( ( ( ( ( ( NOT x3 AND NOT x5 ) AND x4 ) AND NOT x7 ) AND NOT x12 ) OR ( ( ( NOT x3 AND x5 ) AND NOT x7 ) AND NOT x12 ) ) OR ( ( x3 AND NOT x7 ) AND NOT x12 ) )
x13 = ( ( ( ( ( NOT x2 AND x4 ) AND NOT x16 ) AND x11 ) OR ( ( ( ( NOT x2 AND x4 ) AND x16 ) AND x11 ) AND x10 ) ) OR ( ( ( ( x2 AND x4 ) AND NOT x16 ) AND x11 ) AND x10 ) )
x14 = ( ( ( ( NOT x4 AND NOT x7 ) AND x12 ) OR ( NOT x4 AND x7 ) ) OR ( x4 AND x12 ) )
x16 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x15 AND NOT x2 ) AND NOT x4 ) AND NOT x16 ) AND NOT x6 ) AND x14 ) OR ( ( ( ( NOT x15 AND NOT x2 ) AND NOT x4 ) AND NOT x16 ) AND x6 ) ) OR ( ( ( ( ( NOT x15 AND NOT x2 ) AND NOT x4 ) AND x16 ) AND x6 ) AND x14 ) ) OR ( ( ( ( NOT x15 AND NOT x2 ) AND x4 ) AND x6 ) AND x14 ) ) OR ( ( ( NOT x15 AND x2 ) AND NOT x4 ) AND NOT x16 ) ) OR ( ( ( ( ( NOT x15 AND x2 ) AND NOT x4 ) AND x16 ) AND NOT x6 ) AND x14 ) ) OR ( ( ( ( NOT x15 AND x2 ) AND NOT x4 ) AND x16 ) AND x6 ) ) OR ( ( ( ( NOT x15 AND x2 ) AND x4 ) AND NOT x6 ) AND x14 ) ) OR ( ( ( NOT x15 AND x2 ) AND x4 ) AND x6 ) ) OR ( ( ( x15 AND NOT x2 ) AND NOT x4 ) AND NOT x16 ) ) OR ( ( ( ( ( x15 AND NOT x2 ) AND NOT x4 ) AND x16 ) AND NOT x6 ) AND x14 ) ) OR ( ( ( ( x15 AND NOT x2 ) AND NOT x4 ) AND x16 ) AND x6 ) ) OR ( ( ( ( x15 AND NOT x2 ) AND x4 ) AND NOT x6 ) AND x14 ) ) OR ( ( ( x15 AND NOT x2 ) AND x4 ) AND x6 ) ) OR ( x15 AND x2 ) ) \\
LAC-OPERON & 13 & 3 & 10 & x1: v\_A, x2: v\_Am, x3: v\_B, x4: v\_C, x5: v\_Ge, x6: v\_L, x7: v\_Le, x8: v\_Lem, x9: v\_Lm, x10: v\_M, x11: v\_P, x12: v\_R, x13: v\_Rm & x1 = ( x6 AND x3 )
x2 = ( x9 OR x6 )
x3 = x10
x4 = NOT x5
x6 = ( ( x7 AND x11 ) AND NOT x5 )
x9 = ( ( ( x8 AND x11 ) AND NOT x5 ) OR ( x7 AND NOT x5 ) )
x10 = ( x4 AND NOT ( x12 OR x13 ) )
x11 = x10
x12 = NOT ( x2 OR x1 )
x13 = ( x12 OR NOT ( ( x12 OR x2 ) OR x1 ) ) \\
CD4-T-CELL-DIFFERENTIATION-AND-PLASTICITY & 18 & 6 & 12 & x1: v\_BCL6, x2: v\_FOXP3, x3: v\_GATA3, x4: v\_IFNG, x5: v\_IFNGe, x6: v\_IL10, x7: v\_IL10e, x8: v\_IL2, x9: v\_IL21, x10: v\_IL21e, x11: v\_IL2e, x12: v\_IL4, x13: v\_IL4e, x14: v\_IL9, x15: v\_RORGT, x16: v\_TBET, x17: v\_TGFB, x18: v\_TGFBe & x1 = ( x9 AND NOT ( ( x8 OR x16 ) OR x17 ) )
x2 = ( ( x8 AND ( x2 OR x17 ) ) AND NOT ( x9 OR x15 ) )
x3 = ( ( ( x12 AND x8 ) AND NOT ( ( ( ( x16 OR x1 ) OR x17 ) OR x4 ) OR x9 ) ) OR ( x3 AND NOT ( ( ( ( x16 OR x1 ) OR x17 ) OR x4 ) OR x9 ) ) )
x4 = ( ( ( x5 AND NOT ( ( ( x9 OR x12 ) OR x6 ) OR x14 ) ) OR ( x16 AND NOT ( ( ( ( ( ( x9 OR x12 ) OR x1 ) OR x6 ) OR x14 ) OR x17 ) OR x3 ) ) ) OR ( x4 AND NOT ( ( ( ( ( ( x9 OR x12 ) OR x1 ) OR x6 ) OR x14 ) OR x17 ) OR x3 ) ) )
x6 = ( ( x6 AND ( ( ( x3 OR x4 ) OR x9 ) OR x17 ) ) OR x7 )
x8 = ( ( x11 AND NOT ( ( x9 OR x4 ) OR x6 ) ) OR ( x8 AND NOT ( ( ( x9 OR x2 ) OR x4 ) OR x6 ) ) )
x9 = ( ( ( ( x10 AND NOT ( ( ( ( x12 OR x4 ) OR x8 ) OR x14 ) OR x6 ) ) OR ( x1 AND NOT ( ( ( ( x12 OR x4 ) OR x8 ) OR x14 ) OR x6 ) ) ) OR ( x15 AND NOT ( ( ( ( x12 OR x4 ) OR x8 ) OR x14 ) OR x6 ) ) ) OR ( x9 AND NOT ( ( ( ( x12 OR x4 ) OR x8 ) OR x14 ) OR x6 ) ) )
x12 = ( ( x13 AND NOT ( x9 OR x4 ) ) OR ( ( x3 AND ( x8 OR x12 ) ) AND NOT ( ( x16 OR x9 ) OR x4 ) ) )
x14 = ( ( x12 AND ( ( x8 AND x6 ) OR x17 ) ) AND NOT ( x9 OR x4 ) )
x15 = ( ( x9 AND x17 ) AND NOT ( ( ( x16 OR x3 ) OR x1 ) OR x2 ) )
x16 = ( ( x4 AND NOT ( ( ( ( x14 OR x3 ) OR x1 ) OR x9 ) OR x12 ) ) OR ( x16 AND NOT ( ( ( ( x14 OR x3 ) OR x1 ) OR x9 ) OR x12 ) ) )
x17 = ( ( x18 OR ( x2 AND NOT x9 ) ) OR ( x17 AND NOT x9 ) ) \\
HUMAN-GONADAL-SEX-DETERMINATION & 19 & 0 & 19 & x1: v\_AMH, x2: v\_CBX2, x3: v\_CTNNB1, x4: v\_DHH, x5: v\_DKK1, x6: v\_DMRT1, x7: v\_FGF9, x8: v\_FOXL2, x9: v\_GATA4, x10: v\_NR0B1, x11: v\_NR5A1, x12: v\_PGD2, x13: v\_RSPO1, x14: v\_SOX9, x15: v\_SRY, x16: v\_UGR, x17: v\_WNT4, x18: v\_WT1mKTS, x19: v\_WT1pKTS & x1 = ( ( x14 AND ( ( ( x9 AND x18 ) AND x11 ) OR ( x9 AND x11 ) ) ) AND NOT ( x10 AND x3 ) )
x2 = ( x16 AND NOT ( x10 AND ( x17 AND x3 ) ) )
x3 = ( ( x13 AND NOT ( x15 OR ( x14 AND x1 ) ) ) OR ( x17 AND NOT ( x15 OR ( x14 AND x1 ) ) ) )
x4 = x14
x5 = ( x15 OR x14 )
x6 = ( ( x14 AND NOT x8 ) OR ( x15 AND NOT x8 ) )
x7 = ( x14 AND NOT x17 )
x8 = ( ( x17 AND x3 ) AND NOT ( x14 OR x6 ) )
x9 = ( ( ( x15 OR x16 ) OR x17 ) OR x11 )
x10 = ( ( x18 AND NOT ( x11 AND x14 ) ) OR ( ( x17 AND x3 ) AND NOT ( x11 AND x14 ) ) )
x11 = ( ( ( ( x9 AND NOT ( x10 AND x17 ) ) OR ( x16 AND NOT ( x10 AND x17 ) ) ) OR ( x2 AND NOT ( x10 AND x17 ) ) ) OR ( x18 AND NOT ( x10 AND x17 ) ) )
x12 = x14
x13 = ( ( x17 AND NOT x5 ) OR ( x3 AND NOT x5 ) )
x14 = ( ( ( ( ( ( x9 AND ( x15 AND x11 ) ) AND NOT ( ( x3 OR x8 ) OR x17 ) ) OR ( ( x2 AND x15 ) AND NOT ( ( x3 OR x8 ) OR x17 ) ) ) OR ( ( x7 AND x14 ) AND NOT ( ( x3 OR x8 ) OR x17 ) ) ) OR ( x12 AND NOT ( ( x3 OR x8 ) OR x17 ) ) ) OR ( x15 AND NOT ( ( x3 OR x8 ) OR x17 ) ) )
x15 = ( ( ( ( ( x9 AND ( ( x11 AND x2 ) AND x19 ) ) AND NOT x3 ) OR ( x15 AND NOT x3 ) ) OR ( ( x2 AND ( x18 AND x11 ) ) AND NOT x3 ) ) OR ( x14 AND NOT x3 ) )
x16 = ( x16 AND NOT ( x11 OR x17 ) )
x17 = ( ( ( ( x9 AND NOT ( x7 OR x5 ) ) OR ( x3 AND NOT ( x7 OR x5 ) ) ) OR ( x13 AND NOT ( x7 OR x5 ) ) ) OR ( x10 AND NOT ( x7 OR x5 ) ) )
x18 = ( x16 OR x9 )
x19 = ( ( x16 AND NOT ( x17 AND x3 ) ) OR ( x9 AND NOT ( x17 AND x3 ) ) ) \\
COLORECTAL-TUMORIGENESIS-REVERSION-SWITCH & 17 & 0 & 17 & x1: v\_BHLHE40, x2: v\_CDX2, x3: v\_DDIT3, x4: v\_FOSL2, x5: v\_FOXO3, x6: v\_JUN, x7: v\_KLF4, x8: v\_KLF5, x9: v\_KLF6, x10: v\_MAFF, x11: v\_MYC, x12: v\_NFIA, x13: v\_NFIL3, x14: v\_RELB, x15: v\_SMARCA4, x16: v\_SREBF1, x17: v\_YY1 & x1 = ( x9 OR x1 )
x2 = ( x11 OR ( x2 OR x2 ) )
x3 = ( x3 OR ( x8 OR ( x3 OR ( x6 OR ( ( x13 AND x3 ) OR x3 ) ) ) ) )
x4 = ( ( x1 OR x8 ) AND NOT x11 )
x5 = ( x5 AND x6 )
x6 = ( ( x8 AND ( x13 AND NOT x17 ) ) OR ( ( x8 AND ( x3 AND NOT x17 ) ) OR ( ( ( x5 OR x13 ) AND NOT x17 ) OR ( ( ( x8 OR x13 ) AND NOT x17 ) OR ( ( x3 AND ( x13 AND NOT x17 ) ) OR ( ( ( x8 OR x3 ) AND NOT x17 ) OR ( ( x3 AND NOT x17 ) OR ( ( x8 AND NOT x17 ) OR ( ( x13 AND NOT x17 ) OR ( ( ( x3 OR x13 ) AND NOT x17 ) OR ( ( ( x5 OR x3 ) AND NOT x17 ) OR ( ( x8 OR x5 ) AND NOT x17 ) ) ) ) ) ) ) ) ) ) ) )
x7 = ( ( x1 OR x5 ) AND NOT x11 )
x8 = ( ( x6 AND ( x14 AND NOT x17 ) ) OR ( ( x14 AND NOT x17 ) OR ( ( x6 AND NOT x17 ) OR ( ( ( x6 OR x14 ) AND NOT x17 ) OR ( ( ( x5 OR x14 ) AND NOT x17 ) OR ( ( ( x6 OR x5 ) AND NOT x17 ) OR ( ( ( x4 OR x14 ) AND NOT x17 ) OR ( ( x6 OR x4 ) AND NOT x17 ) ) ) ) ) ) ) )
x9 = ( ( x9 AND x10 ) OR x9 )
x10 = ( x5 OR x1 )
x11 = ( x2 OR ( x15 OR x2 ) )
x12 = ( x11 OR ( x16 AND x11 ) )
x13 = ( x3 OR ( x3 OR x6 ) )
x14 = ( x8 OR ( x14 OR x14 ) )
x15 = x11
x16 = ( x17 OR ( x12 OR x17 ) )
x17 = ( x17 OR ( x16 OR ( x17 OR ( x11 OR x17 ) ) ) ) \\
NEUROTRANSMITTER-SIGNALING-PATHWAY & 16 & 2 & 14 & x1: v\_Adenylate\_cyclase, x2: v\_COMT, x3: v\_Calcineurin, x4: v\_Calcium, x5: v\_DARPP32, x6: v\_Dopamine, x7: v\_Dopamine\_Receptor\_1, x8: v\_Dopamine\_Receptor\_2, x9: v\_Exocytosis, x10: v\_Glutamate, x11: v\_Glutamate\_Receptor, x12: v\_Packaging\_Proteins, x13: v\_Phospholipase\_C, x14: v\_Protein\_Kinase\_A, x15: v\_Protein\_Phosphatase\_1, x16: v\_Tryosine\_hydroxylase & x1 = ( x7 AND NOT x8 )
x2 = x6
x3 = x4
x4 = ( x13 OR x11 )
x5 = ( x14 AND NOT x3 )
x6 = ( x16 AND NOT x2 )
x7 = x6
x8 = x6
x9 = x12
x11 = ( ( x14 AND x10 ) AND NOT x15 )
x12 = x11
x13 = x8
x14 = x1
x15 = NOT x5 \\
JNK-PATHWAY & 19 & 6 & 13 & x1: v\_3a, x2: v\_3b, x3: v\_7a, x4: v\_AP\_1\_complex, x5: v\_ATF2\_phosphorylated, x6: v\_Apoptosis\_phenotype, x7: v\_Autophagy\_phenotype, x8: v\_BCL2\_phosphorylated, x9: v\_Innate\_Immunity\_phenotype, x10: v\_MAP2K4\_phosphorylated, x11: v\_MAP2K7\_phosphorylated, x12: v\_MEKK1\_4\_complex, x13: v\_MLK1\_2\_3\_complex, x14: v\_S, x15: v\_SARS\_CoV\_1\_proteins\_complex, x16: v\_TP53\_phosphorylated, x17: v\_TP53\_signalling\_phenotype, x18: v\_csa12\_JNK\_complex\_cell, x19: v\_csa1\_JNK\_complex\_cell & x4 = ( x19 OR x2 )
x5 = x19
x6 = NOT x8
x7 = x8
x8 = x19
x9 = x4
x10 = ( x12 OR x15 )
x11 = ( x13 OR x15 )
x12 = x15
x13 = x15
x16 = x19
x17 = x16
x19 = ( ( ( ( ( x10 OR x11 ) OR x3 ) OR x1 ) AND x18 ) OR ( x18 AND x14 ) ) \\
MIR-9-NEUROGENESIS & 6 & 0 & 6 & x1: v\_Neural\_Precursor, x2: v\_Progenitor, x3: v\_elavl3\_HuC, x4: v\_her6, x5: v\_miR\_9, x6: v\_zic5 & x1 = x3
x2 = ( ( NOT x4 AND x6 ) OR x4 )
x3 = ( NOT x5 AND NOT x2 )
x4 = ( NOT x5 AND NOT x1 )
x5 = ( NOT x4 AND NOT x1 )
x6 = ( NOT x5 AND NOT x1 ) \\
DROSOPHILA-JAK-STAT-PATHWAY & 19 & 12 & 7 & x1: v\_Brwd3, x2: v\_Dome, x3: v\_ET, x4: v\_Hop\_b1, x5: v\_Hop\_b2, x6: v\_Hrs, x7: v\_Ken, x8: v\_NStat92E, x9: v\_OS, x10: v\_Ptp61F, x11: v\_Socs36E, x12: v\_Socs44A, x13: v\_Stam, x14: v\_Stat92E\_b1, x15: v\_Stat92E\_b2, x16: v\_Su\_var, x17: v\_Targets, x18: v\_Upd2, x19: v\_Upd3 & x2 = ( ( ( ( NOT x9 AND NOT x18 ) AND x19 ) OR ( NOT x9 AND x18 ) ) OR x9 )
x4 = ( ( ( ( ( ( ( ( NOT x2 AND x4 ) AND x5 ) OR ( ( ( x2 AND NOT x3 ) AND NOT x6 ) AND NOT x11 ) ) OR ( ( ( ( ( x2 AND NOT x3 ) AND NOT x6 ) AND x11 ) AND x4 ) AND x5 ) ) OR ( ( ( ( x2 AND NOT x3 ) AND x6 ) AND NOT x13 ) AND NOT x11 ) ) OR ( ( ( ( ( ( x2 AND NOT x3 ) AND x6 ) AND NOT x13 ) AND x11 ) AND x4 ) AND x5 ) ) OR ( ( ( x2 AND NOT x3 ) AND x6 ) AND x13 ) ) OR ( ( ( x2 AND x3 ) AND x4 ) AND x5 ) )
x5 = ( ( ( ( ( x2 AND NOT x3 ) AND x6 ) AND x13 ) AND NOT x11 ) AND x4 )
x11 = ( x14 AND x15 )
x14 = ( ( ( ( ( ( ( ( NOT x4 AND x14 ) AND x15 ) OR ( ( ( ( ( x4 AND NOT x12 ) AND NOT x10 ) AND NOT x1 ) AND NOT x7 ) AND NOT x16 ) ) OR ( ( ( ( ( ( ( x4 AND NOT x12 ) AND NOT x10 ) AND NOT x1 ) AND NOT x7 ) AND x16 ) AND x14 ) AND x15 ) ) OR ( ( ( ( ( ( x4 AND NOT x12 ) AND NOT x10 ) AND NOT x1 ) AND x7 ) AND x14 ) AND x15 ) ) OR ( ( ( ( ( x4 AND NOT x12 ) AND NOT x10 ) AND x1 ) AND x14 ) AND x15 ) ) OR ( ( ( ( x4 AND NOT x12 ) AND x10 ) AND x14 ) AND x15 ) ) OR ( ( ( x4 AND x12 ) AND x14 ) AND x15 ) )
x15 = ( ( ( ( ( ( ( x4 AND x5 ) AND NOT x12 ) AND NOT x10 ) AND NOT x1 ) AND NOT x7 ) AND NOT x16 ) AND x14 )
x17 = ( x14 AND NOT x8 ) \\
TUMOUR-CELL-INVASION-AND-MIGRATION-REDUCED & 20 & 2 & 18 & x1: v\_AKT1, x2: v\_AKT2, x3: v\_Apoptosis, x4: v\_CCA, x5: v\_DNAdamage, x6: v\_ECMicroenv, x7: v\_EMT, x8: v\_EMTreg, x9: v\_ERK\_pthw, x10: v\_Ecadh, x11: v\_GF, x12: v\_Invasion, x13: v\_Metastasis, x14: v\_Migration, x15: v\_Notch\_pthw, x16: v\_TGFb\_pthw, x17: v\_WNT\_pthw, x18: v\_miRNA, x19: v\_p53, x20: v\_p63\_73 & x1 = ( ( ( ( ( ( ( ( ( ( NOT x11 AND NOT x16 ) AND NOT x15 ) AND x17 ) AND NOT x19 ) AND x8 ) AND NOT x18 ) AND NOT x10 ) OR ( ( ( ( ( ( NOT x11 AND NOT x16 ) AND x15 ) AND x17 ) AND NOT x19 ) AND NOT x18 ) AND NOT x10 ) ) OR ( ( ( ( ( NOT x11 AND x16 ) AND x17 ) AND NOT x19 ) AND NOT x18 ) AND NOT x10 ) ) OR ( ( ( ( x11 AND x17 ) AND NOT x19 ) AND NOT x18 ) AND NOT x10 ) )
x2 = ( ( NOT x19 AND x8 ) AND NOT x18 )
x3 = ( ( ( ( ( ( ( NOT x19 AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND NOT x9 ) AND x18 ) OR ( ( ( ( NOT x19 AND NOT x8 ) AND x20 ) AND NOT x1 ) AND NOT x9 ) ) OR ( ( ( x19 AND NOT x8 ) AND NOT x1 ) AND NOT x9 ) )
x4 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x16 AND NOT x19 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND NOT x2 ) AND x18 ) OR ( ( ( ( ( ( NOT x16 AND NOT x19 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND x2 ) AND NOT x9 ) ) OR ( ( ( ( ( ( ( NOT x16 AND NOT x19 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND x2 ) AND x9 ) AND x18 ) ) OR ( ( ( ( ( NOT x16 AND NOT x19 ) AND NOT x8 ) AND x20 ) AND NOT x1 ) AND NOT x9 ) ) OR ( ( ( ( ( ( NOT x16 AND NOT x19 ) AND NOT x8 ) AND x20 ) AND NOT x1 ) AND x9 ) AND x18 ) ) OR ( ( ( NOT x16 AND NOT x19 ) AND x8 ) AND NOT x1 ) ) OR ( ( ( ( NOT x16 AND x19 ) AND NOT x8 ) AND NOT x1 ) AND NOT x9 ) ) OR ( ( ( ( ( NOT x16 AND x19 ) AND NOT x8 ) AND NOT x1 ) AND x9 ) AND x18 ) ) OR ( ( ( NOT x16 AND x19 ) AND x8 ) AND NOT x1 ) ) OR ( ( ( ( ( ( ( x16 AND NOT x15 ) AND NOT x19 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND NOT x2 ) AND x18 ) ) OR ( ( ( ( ( ( ( x16 AND NOT x15 ) AND NOT x19 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND x2 ) AND NOT x9 ) ) OR ( ( ( ( ( ( ( ( x16 AND NOT x15 ) AND NOT x19 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND x2 ) AND x9 ) AND x18 ) ) OR ( ( ( ( ( ( x16 AND NOT x15 ) AND NOT x19 ) AND NOT x8 ) AND x20 ) AND NOT x1 ) AND NOT x9 ) ) OR ( ( ( ( ( ( ( x16 AND NOT x15 ) AND NOT x19 ) AND NOT x8 ) AND x20 ) AND NOT x1 ) AND x9 ) AND x18 ) ) OR ( ( ( ( x16 AND NOT x15 ) AND NOT x19 ) AND x8 ) AND NOT x1 ) ) OR ( ( ( ( ( x16 AND NOT x15 ) AND x19 ) AND NOT x8 ) AND NOT x1 ) AND NOT x9 ) ) OR ( ( ( ( ( ( x16 AND NOT x15 ) AND x19 ) AND NOT x8 ) AND NOT x1 ) AND x9 ) AND x18 ) ) OR ( ( ( ( x16 AND NOT x15 ) AND x19 ) AND x8 ) AND NOT x1 ) ) OR ( ( ( ( x16 AND x15 ) AND NOT x8 ) AND NOT x1 ) AND NOT x9 ) ) OR ( ( ( ( ( x16 AND x15 ) AND NOT x8 ) AND NOT x1 ) AND x9 ) AND x18 ) ) OR ( ( ( x16 AND x15 ) AND x8 ) AND NOT x1 ) )
x7 = ( x8 AND NOT x10 )
x8 = ( ( ( ( ( ( NOT x15 AND NOT x17 ) AND NOT x19 ) AND x8 ) AND NOT x18 ) OR ( ( ( NOT x15 AND x17 ) AND NOT x19 ) AND NOT x18 ) ) OR ( ( x15 AND NOT x19 ) AND NOT x18 ) )
x9 = ( ( ( ( ( ( ( NOT x11 AND NOT x16 ) AND NOT x15 ) AND x8 ) AND NOT x1 ) OR ( ( ( NOT x11 AND NOT x16 ) AND x15 ) AND NOT x1 ) ) OR ( ( NOT x11 AND x16 ) AND NOT x1 ) ) OR ( x11 AND NOT x1 ) )
x10 = ( NOT x8 AND NOT x2 )
x11 = ( ( ( NOT x11 AND x8 ) AND NOT x10 ) OR ( x11 AND NOT x10 ) )
x12 = ( ( ( NOT x16 AND x17 ) OR ( ( x16 AND NOT x17 ) AND x8 ) ) OR ( x16 AND x17 ) )
x13 = x14
x14 = ( ( ( ( ( ( x12 AND x7 ) AND NOT x20 ) AND NOT x1 ) AND x2 ) AND x9 ) AND NOT x18 )
x15 = ( ( ( x6 AND NOT x19 ) AND NOT x20 ) AND NOT x18 )
x16 = ( ( ( ( NOT x6 AND x15 ) AND NOT x17 ) AND NOT x18 ) OR ( ( x6 AND NOT x17 ) AND NOT x18 ) )
x17 = ( ( ( ( ( ( ( NOT x15 AND NOT x17 ) AND NOT x19 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND NOT x18 ) AND NOT x10 )
x18 = ( ( ( ( ( NOT x19 AND NOT x8 ) AND x20 ) AND NOT x1 ) AND NOT x2 ) OR ( ( ( x19 AND NOT x8 ) AND NOT x1 ) AND NOT x2 ) )
x19 = ( ( ( ( ( ( ( ( NOT x5 AND NOT x15 ) AND x17 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND NOT x2 ) OR ( ( ( ( ( NOT x5 AND x15 ) AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND NOT x2 ) ) OR ( ( ( ( x5 AND NOT x8 ) AND NOT x20 ) AND NOT x1 ) AND NOT x2 ) )
x20 = ( ( ( ( ( x5 AND NOT x15 ) AND NOT x19 ) AND NOT x8 ) AND NOT x1 ) AND NOT x2 ) \\
P53-MDM2-NETWORK & 6 & 1 & 5 & x1: v\_DNAdam, x2: v\_Mdm2cyt\_b1, x3: v\_Mdm2cyt\_b2, x4: v\_Mdm2nuc, x5: v\_p53\_b1, x6: v\_p53\_b2 & x1 = ( ( NOT x5 AND x1 ) OR ( ( x5 AND NOT x6 ) AND x1 ) )
x3 = ( ( x5 AND x6 ) AND x2 )
x4 = ( ( ( ( ( NOT x5 AND x2 ) AND NOT x3 ) AND NOT x1 ) OR ( ( NOT x5 AND x2 ) AND x3 ) ) OR ( ( x5 AND x2 ) AND x3 ) )
x5 = ( ( ( NOT x5 AND NOT x4 ) OR ( ( x5 AND NOT x6 ) AND NOT x4 ) ) OR ( x5 AND x6 ) )
x6 = ( x5 AND NOT x4 ) \\
DROSOPHILA-GAP-A & 7 & 2 & 5 & x1: v\_Gt, x2: v\_Hb\_b1, x3: v\_Hb\_b2, x4: v\_Hb\_b3, x5: v\_Kni, x6: v\_Kr\_b1, x7: v\_Kr\_b2 & x1 = NOT x6
x3 = x2
x4 = ( x2 AND x3 )
x6 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x1 AND NOT x2 ) AND x6 ) AND x7 ) OR ( ( NOT x1 AND x2 ) AND NOT x3 ) ) OR ( ( ( NOT x1 AND x2 ) AND x3 ) AND NOT x4 ) ) OR ( ( ( ( ( NOT x1 AND x2 ) AND x3 ) AND x4 ) AND x6 ) AND x7 ) ) OR ( ( ( x1 AND NOT x2 ) AND x6 ) AND x7 ) ) OR ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND NOT x6 ) AND NOT x5 ) ) OR ( ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND x6 ) AND NOT x7 ) AND NOT x5 ) ) OR ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND x6 ) AND x7 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND NOT x6 ) AND NOT x5 ) ) OR ( ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND NOT x7 ) AND NOT x5 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND x7 ) ) OR ( ( ( ( ( x1 AND x2 ) AND x3 ) AND x4 ) AND x6 ) AND x7 ) )
x7 = ( ( ( ( ( NOT x1 AND x2 ) AND NOT x3 ) AND x6 ) AND NOT x5 ) OR ( ( ( ( ( NOT x1 AND x2 ) AND x3 ) AND NOT x4 ) AND x6 ) AND NOT x5 ) ) \\
TOLL-PATHWAY-OF-DROSOPHILA & 11 & 2 & 9 & x1: v\_Cactus, x2: v\_Dif, x3: v\_Dorsal, x4: v\_MyD88, x5: v\_Nec, x6: v\_Pelle, x7: v\_Slmb, x8: v\_Spz, x9: v\_Targets, x10: v\_Toll, x11: v\_Tube & x1 = NOT ( x6 AND x7 )
x2 = NOT x1
x3 = NOT x1
x4 = x10
x6 = x11
x8 = NOT x5
x9 = ( x3 OR x2 )
x10 = x8
x11 = x4 \\
SEGMENT-POLARITY-1-CELL & 19 & 2 & 17 & x1: v\_Ci1, x2: v\_Ciact\_b1, x3: v\_Ciact\_b2, x4: v\_Cirep, x5: v\_Dsh, x6: v\_En, x7: v\_Fz, x8: v\_Hh, x9: v\_Hh\_ext, x10: v\_Nkd\_b1, x11: v\_Nkd\_b2, x12: v\_Pka\_b1, x13: v\_Pka\_b2, x14: v\_Ptc\_b1, x15: v\_Ptc\_b2, x16: v\_Slp, x17: v\_Wg\_b1, x18: v\_Wg\_b2, x19: v\_Wg\_ext & x1 = NOT x6
x2 = ( ( ( ( ( ( ( ( NOT x5 AND NOT x1 ) AND x2 ) AND x3 ) OR ( ( ( NOT x5 AND x1 ) AND NOT x2 ) AND NOT x12 ) ) OR ( ( ( ( NOT x5 AND x1 ) AND x2 ) AND NOT x3 ) AND NOT x12 ) ) OR ( ( ( NOT x5 AND x1 ) AND x2 ) AND x3 ) ) OR ( ( ( x5 AND NOT x1 ) AND x2 ) AND x3 ) ) OR ( x5 AND x1 ) )
x3 = ( ( ( x5 AND x1 ) AND x2 ) AND NOT x12 )
x4 = ( ( ( NOT x5 AND x1 ) AND x12 ) AND x13 )
x5 = x7
x6 = ( x5 AND NOT x16 )
x7 = ( ( NOT x17 AND x19 ) OR x17 )
x8 = ( x6 AND NOT x4 )
x10 = ( ( ( NOT x10 AND NOT x6 ) OR ( ( x10 AND NOT x11 ) AND NOT x6 ) ) OR ( x10 AND x11 ) )
x11 = ( ( x5 AND x10 ) AND NOT x6 )
x12 = ( ( ( NOT x12 AND x14 ) OR ( ( x12 AND NOT x13 ) AND x14 ) ) OR ( x12 AND x13 ) )
x13 = ( x12 AND x14 )
x14 = ( ( ( ( ( NOT x6 AND NOT x14 ) AND NOT x9 ) OR ( ( ( NOT x6 AND x14 ) AND NOT x15 ) AND NOT x9 ) ) OR ( ( NOT x6 AND x14 ) AND x15 ) ) OR ( ( x6 AND x14 ) AND x15 ) )
x15 = ( ( ( NOT x6 AND x2 ) AND x14 ) AND NOT x9 )
x16 = ( x5 AND NOT x6 )
x17 = ( ( ( ( ( ( ( ( ( ( NOT x17 AND x16 ) AND NOT x10 ) AND NOT x6 ) AND x2 ) OR ( ( ( ( ( NOT x17 AND x16 ) AND x10 ) AND NOT x11 ) AND NOT x6 ) AND x2 ) ) OR ( ( ( ( ( ( NOT x17 AND x16 ) AND x10 ) AND x11 ) AND NOT x6 ) AND x2 ) AND x3 ) ) OR ( ( ( ( ( x17 AND NOT x18 ) AND x16 ) AND NOT x10 ) AND NOT x6 ) AND x2 ) ) OR ( ( ( ( ( ( x17 AND NOT x18 ) AND x16 ) AND x10 ) AND NOT x11 ) AND NOT x6 ) AND x2 ) ) OR ( ( ( ( ( ( ( x17 AND NOT x18 ) AND x16 ) AND x10 ) AND x11 ) AND NOT x6 ) AND x2 ) AND x3 ) ) OR ( x17 AND x18 ) )
x18 = ( ( ( ( x17 AND x16 ) AND NOT x6 ) AND x2 ) AND x3 ) \\
BT474-BREAST-CELL-LINE-SHORT-TERM & 16 & 5 & 11 & x1: v\_AKT, x2: v\_EGF, x3: v\_ERBB1, x4: v\_ERBB2, x5: v\_ERBB3, x6: v\_ERK1\_2, x7: v\_HRG, x8: v\_MEK1\_2, x9: v\_PDK1, x10: v\_PKCa, x11: v\_PLCg, x12: v\_erlotinib, x13: v\_mTOR, x14: v\_p70S6K, x15: v\_pertuzumab, x16: v\_trastuzumab & x1 = ( ( ( x5 OR x9 ) OR x13 ) OR x1 )
x3 = ( ( ( x3 AND NOT ( x12 OR x15 ) ) OR ( x2 AND NOT ( x12 OR x15 ) ) ) OR ( x11 AND NOT ( x12 OR x15 ) ) )
x4 = ( ( ( x5 AND NOT ( ( x12 OR x16 ) OR x15 ) ) OR ( x4 AND NOT ( ( x12 OR x16 ) OR x15 ) ) ) OR ( x2 AND NOT ( ( x12 OR x16 ) OR x15 ) ) )
x5 = ( ( x7 AND NOT ( ( x15 OR x15 ) OR x12 ) ) OR ( x5 AND NOT ( ( x15 OR x15 ) OR x12 ) ) )
x6 = ( ( ( x8 OR x6 ) OR x15 ) OR x2 )
x8 = ( ( ( x5 OR x3 ) OR x8 ) OR x4 )
x9 = ( ( ( ( x3 OR x9 ) OR x5 ) OR x8 ) OR x4 )
x10 = ( x11 OR x10 )
x11 = ( ( ( ( x3 OR x11 ) OR x4 ) OR x5 ) OR x2 )
x13 = ( ( x1 OR x13 ) OR x15 )
x14 = ( ( ( x14 OR x1 ) OR x6 ) OR x13 ) \\
PAIR-RULE-MODULE & 11 & 0 & 11 & x1: v\_Eve\_b1, x2: v\_Eve\_b2, x3: v\_Eve\_b3, x4: v\_Ftz\_b1, x5: v\_Ftz\_b2, x6: v\_Odd, x7: v\_Ppa, x8: v\_Prd\_b1, x9: v\_Prd\_b2, x10: v\_Run, x11: v\_Slp & x1 = ( ( ( ( ( ( NOT x1 AND x8 ) AND NOT x11 ) AND NOT x6 ) OR ( ( ( x1 AND NOT x2 ) AND NOT x10 ) AND NOT x11 ) ) OR ( ( ( ( x1 AND NOT x2 ) AND x10 ) AND NOT x11 ) AND NOT x6 ) ) OR ( x1 AND x2 ) )
x2 = ( ( ( ( ( ( ( x1 AND NOT x2 ) AND x8 ) AND NOT x10 ) AND NOT x11 ) AND NOT x6 ) OR ( ( ( ( ( ( x1 AND x2 ) AND NOT x3 ) AND x8 ) AND NOT x10 ) AND NOT x11 ) AND NOT x6 ) ) OR ( ( x1 AND x2 ) AND x3 ) )
x3 = ( ( ( ( ( x1 AND x2 ) AND x8 ) AND NOT x10 ) AND NOT x11 ) AND NOT x6 )
x4 = ( ( ( ( ( ( ( ( ( ( ( NOT x1 AND NOT x11 ) AND NOT x4 ) AND NOT x6 ) OR ( ( ( ( NOT x1 AND NOT x11 ) AND x4 ) AND NOT x5 ) AND NOT x6 ) ) OR ( ( ( NOT x1 AND NOT x11 ) AND x4 ) AND x5 ) ) OR ( ( ( NOT x1 AND x11 ) AND x4 ) AND x5 ) ) OR ( ( ( ( x1 AND NOT x2 ) AND NOT x11 ) AND NOT x4 ) AND NOT x6 ) ) OR ( ( ( ( ( x1 AND NOT x2 ) AND NOT x11 ) AND x4 ) AND NOT x5 ) AND NOT x6 ) ) OR ( ( ( ( x1 AND NOT x2 ) AND NOT x11 ) AND x4 ) AND x5 ) ) OR ( ( ( ( x1 AND NOT x2 ) AND x11 ) AND x4 ) AND x5 ) ) OR ( ( ( x1 AND x2 ) AND x4 ) AND x5 ) )
x5 = ( ( ( ( NOT x1 AND NOT x11 ) AND x4 ) AND NOT x6 ) OR ( ( ( ( x1 AND NOT x2 ) AND NOT x11 ) AND x4 ) AND NOT x6 ) )
x6 = ( NOT x1 AND NOT x8 )
x7 = ( NOT x1 OR ( x1 AND NOT x2 ) )
x8 = ( ( ( NOT x8 AND NOT x6 ) OR ( ( x8 AND NOT x9 ) AND NOT x6 ) ) OR ( x8 AND x9 ) )
x9 = ( ( x8 AND NOT x7 ) AND NOT x6 )
x10 = ( ( ( NOT x1 AND x8 ) AND NOT x6 ) OR ( ( ( x1 AND NOT x2 ) AND x8 ) AND NOT x6 ) )
x11 = ( ( ( NOT x1 AND NOT x4 ) AND NOT x6 ) OR ( ( ( x1 AND NOT x2 ) AND NOT x4 ) AND NOT x6 ) ) \\
BUDDING-YEAST-CELL-CYCLE & 20 & 4 & 16 & x1: v\_BuddingCP, x2: v\_Cdc14, x3: v\_Cdc20, x4: v\_Cdh1, x5: v\_Clb2, x6: v\_Clb5, x7: v\_Cln2, x8: v\_Cln3, x9: v\_FEAR, x10: v\_MEN, x11: v\_SFF, x12: v\_SMBF, x13: v\_Sic1, x14: v\_Size, x15: v\_SpindleCP, x16: v\_Start, x17: v\_Swe1, x18: v\_Swi5, x19: v\_Whi5, x20: v\_Yhp1 & x2 = ( x10 AND x9 )
x3 = ( x15 AND ( x5 AND x11 ) )
x4 = ( x2 OR NOT ( ( ( x6 OR x2 ) OR x5 ) OR x7 ) )
x5 = ( ( x11 AND NOT ( ( ( x4 AND x3 ) OR ( x3 AND x4 ) ) OR x17 ) ) OR NOT ( ( ( ( x17 OR x11 ) OR x4 ) OR x3 ) OR x13 ) )
x6 = ( x12 AND NOT ( x13 OR x3 ) )
x7 = ( x12 AND x16 )
x8 = ( x14 AND NOT x20 )
x9 = x3
x10 = ( x9 AND x5 )
x11 = x5
x12 = ( NOT ( x5 OR x19 ) OR NOT ( x19 OR x5 ) )
x13 = ( ( ( x18 AND NOT ( ( ( x6 AND NOT x2 ) OR ( x5 AND NOT x2 ) ) OR ( x7 AND NOT x2 ) ) ) OR ( x13 AND NOT ( ( ( x6 AND NOT x2 ) OR ( x5 AND NOT x2 ) ) OR ( x7 AND NOT x2 ) ) ) ) OR NOT ( ( ( ( ( x18 OR x6 ) OR x2 ) OR x5 ) OR x7 ) OR x13 ) )
x17 = ( NOT x1 OR NOT x1 )
x18 = ( ( x2 AND ( x11 AND NOT x18 ) ) AND NOT x5 )
x19 = ( NOT ( ( x7 AND x16 ) OR ( x8 AND x16 ) ) OR NOT ( ( x16 OR x8 ) OR x7 ) )
x20 = x12 \\
AGS-CELL-FATE-DECISION-REDUCED & 14 & 2 & 12 & x1: v\_AKT, x2: v\_Antisurvival\_b1, x3: v\_Antisurvival\_b2, x4: v\_Antisurvival\_b3, x5: v\_ERK, x6: v\_GSK3, x7: v\_MEK, x8: v\_PI3K, x9: v\_Prosurvival\_b1, x10: v\_Prosurvival\_b2, x11: v\_Prosurvival\_b3, x12: v\_TAK1, x13: v\_betacatenin, x14: v\_p38alpha & x1 = ( ( ( ( ( ( ( ( ( ( ( NOT x5 AND NOT x12 ) AND NOT x1 ) AND NOT x8 ) AND x6 ) OR ( ( ( NOT x5 AND NOT x12 ) AND NOT x1 ) AND x8 ) ) OR ( ( ( NOT x5 AND NOT x12 ) AND x1 ) AND x8 ) ) OR ( ( ( ( NOT x5 AND x12 ) AND x8 ) AND NOT x6 ) AND x13 ) ) OR ( ( ( NOT x5 AND x12 ) AND x8 ) AND x6 ) ) OR ( ( x5 AND NOT x12 ) AND x8 ) ) OR ( ( ( ( x5 AND x12 ) AND x8 ) AND NOT x6 ) AND x13 ) ) OR ( ( ( x5 AND x12 ) AND x8 ) AND x6 ) )
x2 = ( ( ( ( ( NOT x5 AND NOT x14 ) OR ( ( NOT x5 AND x14 ) AND NOT x1 ) ) OR ( ( ( ( NOT x5 AND x14 ) AND x1 ) AND x2 ) AND x3 ) ) OR ( x5 AND NOT x1 ) ) OR ( ( ( x5 AND x1 ) AND x2 ) AND x3 ) )
x3 = ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x5 AND NOT x12 ) AND NOT x1 ) AND x2 ) OR ( ( ( ( ( NOT x5 AND NOT x12 ) AND x1 ) AND x2 ) AND x3 ) AND x4 ) ) OR ( ( ( ( ( NOT x5 AND x12 ) AND NOT x14 ) AND x2 ) AND x3 ) AND x4 ) ) OR ( ( ( ( ( ( ( NOT x5 AND x12 ) AND x14 ) AND NOT x1 ) AND NOT x8 ) AND x2 ) AND x3 ) AND x4 ) ) OR ( ( ( ( ( ( ( ( ( NOT x5 AND x12 ) AND x14 ) AND NOT x1 ) AND x8 ) AND NOT x6 ) AND NOT x13 ) AND x2 ) AND x3 ) AND x4 ) ) OR ( ( ( ( ( ( ( NOT x5 AND x12 ) AND x14 ) AND NOT x1 ) AND x8 ) AND NOT x6 ) AND x13 ) AND x2 ) ) OR ( ( ( ( ( ( NOT x5 AND x12 ) AND x14 ) AND NOT x1 ) AND x8 ) AND x6 ) AND x2 ) ) OR ( ( ( ( ( ( NOT x5 AND x12 ) AND x14 ) AND x1 ) AND x2 ) AND x3 ) AND x4 ) ) OR ( ( ( x5 AND NOT x12 ) AND NOT x1 ) AND x2 ) ) OR ( ( ( ( ( x5 AND NOT x12 ) AND x1 ) AND x2 ) AND x3 ) AND x4 ) ) OR ( ( ( ( x5 AND x12 ) AND x2 ) AND x3 ) AND x4 ) )
x4 = ( ( ( ( ( ( NOT x5 AND NOT x12 ) AND x14 ) AND NOT x1 ) AND x8 ) AND x2 ) AND x3 )
x5 = ( ( ( NOT x7 AND NOT x5 ) AND NOT x1 ) OR x7 )
x7 = ( ( ( ( ( NOT x5 OR ( x5 AND NOT x12 ) ) OR ( ( x5 AND x12 ) AND NOT x14 ) ) OR ( ( ( x5 AND x12 ) AND x14 ) AND NOT x1 ) ) OR ( ( ( ( ( x5 AND x12 ) AND x14 ) AND x1 ) AND NOT x6 ) AND x13 ) ) OR ( ( ( ( x5 AND x12 ) AND x14 ) AND x1 ) AND x6 ) )
x8 = ( ( ( NOT x5 OR ( x5 AND NOT x12 ) ) OR ( ( ( x5 AND x12 ) AND NOT x6 ) AND x13 ) ) OR ( ( x5 AND x12 ) AND x6 ) )
x9 = ( ( ( ( ( ( ( ( ( NOT x5 AND NOT x12 ) OR ( ( ( ( NOT x5 AND x12 ) AND NOT x13 ) AND x9 ) AND x10 ) ) OR ( ( NOT x5 AND x12 ) AND x13 ) ) OR ( x5 AND NOT x12 ) ) OR ( ( ( ( ( x5 AND x12 ) AND NOT x8 ) AND NOT x13 ) AND x9 ) AND x10 ) ) OR ( ( ( x5 AND x12 ) AND NOT x8 ) AND x13 ) ) OR ( ( ( ( ( ( x5 AND x12 ) AND x8 ) AND NOT x6 ) AND NOT x13 ) AND x9 ) AND x10 ) ) OR ( ( ( ( x5 AND x12 ) AND x8 ) AND NOT x6 ) AND x13 ) ) OR ( ( ( x5 AND x12 ) AND x8 ) AND x6 ) )
x10 = ( ( ( NOT x12 AND x9 ) OR ( ( ( ( x12 AND NOT x13 ) AND x9 ) AND x10 ) AND x11 ) ) OR ( ( x12 AND x13 ) AND x9 ) )
x11 = ( ( ( ( ( x5 AND NOT x12 ) AND x8 ) AND x9 ) AND x10 ) OR ( ( ( ( ( x5 AND x12 ) AND x8 ) AND x13 ) AND x9 ) AND x10 ) )
x12 = NOT x14
x14 = ( NOT x5 AND NOT x14 ) \\
HEMATOPOIESIS-AGING & 15 & 0 & 15 & x1: v\_Bclaf1, x2: v\_CDK46CycD, x3: v\_CIPKIP, x4: v\_Cebpa, x5: v\_Egr1, x6: v\_Fli1, x7: v\_Gata1, x8: v\_Gata2, x9: v\_Ikzf1, x10: v\_Junb, x11: v\_Klf1, x12: v\_Myc, x13: v\_Spi1, x14: v\_Tal1, x15: v\_Zfpm1 & x1 = x12
x2 = ( x1 OR x12 )
x3 = x10
x4 = ( ( x8 AND NOT x9 ) OR ( x13 AND NOT x9 ) )
x5 = ( x8 AND x10 )
x6 = ( x10 OR ( x7 AND NOT x11 ) )
x7 = ( x6 OR ( ( x8 AND NOT x13 ) OR ( x7 AND ( NOT x9 AND NOT x13 ) ) ) )
x8 = ( ( x8 AND ( NOT x7 AND NOT x15 ) ) OR ( x5 AND ( NOT x7 AND ( NOT x15 AND NOT x13 ) ) ) )
x9 = x8
x10 = ( x5 OR x12 )
x11 = ( x7 AND NOT x6 )
x12 = ( x4 AND x1 )
x13 = ( ( x13 AND NOT x7 ) OR ( x4 AND ( NOT x7 AND NOT x8 ) ) )
x14 = ( x7 AND NOT x13 )
x15 = x7 \\
BOOLEAN-CELL-CYCLE & 14 & 2 & 12 & x1: v\_Cdc20, x2: v\_Cdh1, x3: v\_CycA, x4: v\_CycB, x5: v\_CycD, x6: v\_CycE, x7: v\_E2F, x8: v\_Rb1, x9: v\_Rb2, x10: v\_Skp2, x11: v\_UbcH10, x12: v\_p27\_1\_b1, x13: v\_p27\_1\_b2, x14: v\_p27\_2 & x1 = x4
x2 = ( ( ( ( NOT x3 AND NOT x4 ) OR ( ( NOT x3 AND x4 ) AND x12 ) ) OR ( ( x3 AND x12 ) AND NOT x10 ) ) OR ( ( ( x3 AND x12 ) AND x10 ) AND x14 ) )
x3 = ( ( ( ( ( ( ( ( ( ( ( NOT x7 AND x3 ) AND NOT x1 ) AND NOT x2 ) OR ( ( ( ( NOT x7 AND x3 ) AND NOT x1 ) AND x2 ) AND NOT x11 ) ) OR ( ( ( NOT x7 AND x3 ) AND x1 ) AND NOT x11 ) ) OR ( ( ( ( x7 AND NOT x3 ) AND NOT x1 ) AND NOT x2 ) AND NOT x8 ) ) OR ( ( ( ( ( x7 AND NOT x3 ) AND NOT x1 ) AND x2 ) AND NOT x11 ) AND NOT x8 ) ) OR ( ( ( ( x7 AND NOT x3 ) AND x1 ) AND NOT x11 ) AND NOT x8 ) ) OR ( ( ( x7 AND x3 ) AND NOT x1 ) AND NOT x2 ) ) OR ( ( ( ( x7 AND x3 ) AND NOT x1 ) AND x2 ) AND NOT x11 ) ) OR ( ( ( x7 AND x3 ) AND x1 ) AND NOT x11 ) )
x4 = ( ( NOT x1 AND NOT x2 ) OR ( ( x1 AND NOT x2 ) AND NOT x11 ) )
x6 = ( ( NOT x9 AND x7 ) OR ( ( x9 AND x7 ) AND NOT x8 ) )
x7 = ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x9 AND NOT x3 ) AND NOT x4 ) OR ( ( ( NOT x9 AND NOT x3 ) AND x4 ) AND NOT x1 ) ) OR ( ( ( NOT x9 AND x3 ) AND NOT x4 ) AND NOT x10 ) ) OR ( ( ( ( NOT x9 AND x3 ) AND NOT x4 ) AND x10 ) AND x14 ) ) OR ( ( ( ( NOT x9 AND x3 ) AND x4 ) AND NOT x1 ) AND NOT x10 ) ) OR ( ( ( ( ( NOT x9 AND x3 ) AND x4 ) AND NOT x1 ) AND x10 ) AND x14 ) ) OR ( ( ( x9 AND NOT x3 ) AND NOT x4 ) AND NOT x8 ) ) OR ( ( ( ( x9 AND NOT x3 ) AND x4 ) AND NOT x1 ) AND NOT x8 ) ) OR ( ( ( ( x9 AND x3 ) AND NOT x4 ) AND NOT x10 ) AND NOT x8 ) ) OR ( ( ( ( ( x9 AND x3 ) AND NOT x4 ) AND x10 ) AND NOT x8 ) AND x14 ) ) OR ( ( ( ( ( x9 AND x3 ) AND x4 ) AND NOT x1 ) AND NOT x10 ) AND NOT x8 ) ) OR ( ( ( ( ( ( x9 AND x3 ) AND x4 ) AND NOT x1 ) AND x10 ) AND NOT x8 ) AND x14 ) )
x8 = ( ( ( ( ( ( ( NOT x9 AND NOT x6 ) AND NOT x3 ) AND NOT x4 ) OR ( ( ( ( NOT x9 AND NOT x6 ) AND NOT x3 ) AND x4 ) AND x12 ) ) OR ( ( ( NOT x9 AND NOT x6 ) AND x3 ) AND x12 ) ) OR ( ( NOT x9 AND x6 ) AND x12 ) ) OR x9 )
x9 = ( ( ( ( ( ( ( ( NOT x5 AND NOT x6 ) AND NOT x3 ) AND NOT x4 ) AND x8 ) OR ( ( ( ( ( NOT x5 AND NOT x6 ) AND NOT x3 ) AND x4 ) AND x12 ) AND x8 ) ) OR ( ( ( ( NOT x5 AND NOT x6 ) AND x3 ) AND x12 ) AND x8 ) ) OR ( ( ( ( NOT x5 AND x6 ) AND NOT x3 ) AND x12 ) AND x8 ) ) OR ( ( ( ( ( NOT x5 AND x6 ) AND x3 ) AND NOT x4 ) AND x12 ) AND x8 ) )
x10 = ( ( NOT x9 OR ( x9 AND NOT x2 ) ) OR ( ( x9 AND x2 ) AND NOT x8 ) )
x11 = ( ( ( ( ( ( ( ( ( NOT x3 AND NOT x4 ) AND NOT x1 ) AND NOT x2 ) OR ( ( ( NOT x3 AND NOT x4 ) AND x1 ) AND NOT x2 ) ) OR ( ( ( ( NOT x3 AND NOT x4 ) AND x1 ) AND x2 ) AND x11 ) ) OR ( ( NOT x3 AND x4 ) AND NOT x2 ) ) OR ( ( ( NOT x3 AND x4 ) AND x2 ) AND x11 ) ) OR ( x3 AND NOT x2 ) ) OR ( ( x3 AND x2 ) AND x11 ) )
x12 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x5 AND NOT x12 ) AND x14 ) OR ( ( ( NOT x5 AND x12 ) AND NOT x13 ) AND x14 ) ) OR ( ( NOT x5 AND x12 ) AND x13 ) ) OR ( ( ( x5 AND NOT x6 ) AND NOT x3 ) AND NOT x4 ) ) OR ( ( ( ( ( x5 AND NOT x6 ) AND NOT x3 ) AND x4 ) AND NOT x12 ) AND NOT x10 ) ) OR ( ( ( ( ( ( x5 AND NOT x6 ) AND NOT x3 ) AND x4 ) AND NOT x12 ) AND x10 ) AND x14 ) ) OR ( ( ( ( ( ( x5 AND NOT x6 ) AND NOT x3 ) AND x4 ) AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( ( ( ( ( ( x5 AND NOT x6 ) AND NOT x3 ) AND x4 ) AND x12 ) AND NOT x13 ) AND x10 ) AND x14 ) ) OR ( ( ( ( ( x5 AND NOT x6 ) AND NOT x3 ) AND x4 ) AND x12 ) AND x13 ) ) OR ( ( ( ( ( x5 AND NOT x6 ) AND x3 ) AND NOT x4 ) AND NOT x12 ) AND NOT x10 ) ) OR ( ( ( ( ( ( x5 AND NOT x6 ) AND x3 ) AND NOT x4 ) AND NOT x12 ) AND x10 ) AND x14 ) ) OR ( ( ( ( x5 AND NOT x6 ) AND x3 ) AND NOT x4 ) AND x12 ) ) OR ( ( ( ( ( x5 AND NOT x6 ) AND x3 ) AND x4 ) AND NOT x12 ) AND NOT x10 ) ) OR ( ( ( ( ( ( x5 AND NOT x6 ) AND x3 ) AND x4 ) AND NOT x12 ) AND x10 ) AND x14 ) ) OR ( ( ( ( ( ( x5 AND NOT x6 ) AND x3 ) AND x4 ) AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( ( ( ( ( ( x5 AND NOT x6 ) AND x3 ) AND x4 ) AND x12 ) AND NOT x13 ) AND x10 ) AND x14 ) ) OR ( ( ( ( ( x5 AND NOT x6 ) AND x3 ) AND x4 ) AND x12 ) AND x13 ) ) OR ( ( ( x5 AND x6 ) AND NOT x12 ) AND NOT x10 ) ) OR ( ( ( ( x5 AND x6 ) AND NOT x12 ) AND x10 ) AND x14 ) ) OR ( ( ( ( x5 AND x6 ) AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( ( ( ( x5 AND x6 ) AND x12 ) AND NOT x13 ) AND x10 ) AND x14 ) ) OR ( ( ( x5 AND x6 ) AND x12 ) AND x13 ) )
x14 = ( ( ( ( ( ( ( ( NOT x5 AND NOT x6 ) AND NOT x4 ) AND x12 ) OR ( ( ( ( NOT x5 AND NOT x6 ) AND x4 ) AND x12 ) AND NOT x10 ) ) OR ( ( ( ( ( NOT x5 AND x6 ) AND NOT x3 ) AND NOT x4 ) AND x12 ) AND NOT x10 ) ) OR ( ( ( ( ( ( NOT x5 AND x6 ) AND NOT x3 ) AND NOT x4 ) AND x12 ) AND x10 ) AND x14 ) ) OR ( ( ( ( ( NOT x5 AND x6 ) AND NOT x3 ) AND x4 ) AND x12 ) AND NOT x10 ) ) OR ( ( ( ( NOT x5 AND x6 ) AND x3 ) AND x12 ) AND NOT x10 ) ) \\
CELL-CYCLE-TRANSCRIPTION & 9 & 0 & 9 & x1: v\_ACE2, x2: v\_CLN3, x3: v\_HCM1, x4: v\_MBF, x5: v\_SBF, x6: v\_SFF, x7: v\_SWI5, x8: v\_YHP1, x9: v\_YOX1 & x1 = x6
x2 = ( ( x7 AND x1 ) AND NOT ( x9 OR x8 ) )
x3 = ( x4 AND x5 )
x4 = x2
x5 = ( ( x4 AND NOT ( x8 OR x9 ) ) OR ( x2 AND NOT ( x8 OR x9 ) ) )
x6 = ( x5 AND x3 )
x7 = x6
x8 = ( x5 OR x4 )
x9 = ( x4 AND x5 ) \\
ARABIDOPSIS-THALIANA-CELL-CYCLE & 14 & 0 & 14 & x1: v\_APC\_C, x2: v\_CDKB1\_1, x3: v\_CYCA2\_3, x4: v\_CYCB1\_1, x5: v\_CYCD3\_1, x6: v\_E2Fa, x7: v\_E2Fb, x8: v\_E2Fc, x9: v\_E2Fe, x10: v\_KRP1, x11: v\_MYB3R1\_4, x12: v\_MYB77, x13: v\_RBR, x14: v\_SCF & x1 = ( ( ( x12 AND NOT x9 ) OR ( x11 AND NOT x9 ) ) OR ( x6 AND NOT ( x9 OR x13 ) ) )
x2 = ( ( x12 OR ( ( x7 AND ( NOT x13 OR ( x5 AND NOT x10 ) ) ) AND NOT x8 ) ) OR x11 )
x3 = ( ( x11 AND NOT x1 ) OR ( x12 AND NOT x1 ) )
x4 = ( ( ( x11 AND NOT x1 ) OR ( ( x7 AND ( ( x5 AND NOT x10 ) OR NOT x13 ) ) AND NOT ( x1 OR x8 ) ) ) OR ( x12 AND NOT x1 ) )
x5 = NOT x14
x6 = ( ( ( ( x2 AND ( ( NOT x8 AND NOT x3 ) AND NOT x6 ) ) OR ( x3 AND ( ( NOT x8 AND NOT x2 ) AND NOT x6 ) ) ) OR ( x6 AND NOT ( x2 AND x3 ) ) ) OR NOT ( ( ( x8 OR x2 ) OR x3 ) OR x6 ) )
x7 = ( x6 AND NOT x13 )
x8 = ( ( x11 AND NOT ( ( x14 AND x5 ) AND NOT x10 ) ) OR ( x6 AND NOT ( x13 OR ( ( x14 AND x5 ) AND NOT x10 ) ) ) )
x9 = ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( ( x7 AND ( NOT x13 OR ( NOT x10 AND x5 ) ) ) OR x12 ) OR ( x5 AND ( ( ( ( NOT x10 AND NOT x12 ) AND NOT x8 ) AND NOT x7 ) AND NOT x13 ) ) ) OR ( x13 AND ( ( ( ( NOT x10 AND NOT x12 ) AND NOT x8 ) AND NOT x5 ) AND NOT x7 ) ) ) OR ( ( x5 AND ( x7 AND x13 ) ) AND ( ( NOT x10 AND NOT x12 ) AND NOT x8 ) ) ) OR ( ( x5 AND ( x10 AND x7 ) ) AND ( ( NOT x12 AND NOT x8 ) AND NOT x13 ) ) ) OR ( ( x5 AND x10 ) AND ( ( ( NOT x12 AND NOT x8 ) AND NOT x7 ) AND NOT x13 ) ) ) OR ( x10 AND ( ( ( ( NOT x12 AND NOT x8 ) AND NOT x5 ) AND NOT x7 ) AND NOT x13 ) ) ) OR ( ( x13 AND x10 ) AND ( ( ( NOT x12 AND NOT x8 ) AND NOT x5 ) AND NOT x7 ) ) ) OR ( ( x5 AND x13 ) AND ( ( ( NOT x10 AND NOT x12 ) AND NOT x8 ) AND NOT x7 ) ) ) OR ( ( x7 AND ( x10 AND x13 ) ) AND ( ( NOT x12 AND NOT x8 ) AND NOT x5 ) ) ) OR ( ( x7 AND ( x10 AND x8 ) ) AND ( ( NOT x12 AND NOT x5 ) AND NOT x13 ) ) ) OR ( ( x5 AND ( ( x10 AND x7 ) AND x13 ) ) AND ( NOT x12 AND NOT x8 ) ) ) OR ( ( x7 AND x10 ) AND ( ( ( NOT x12 AND NOT x8 ) AND NOT x5 ) AND NOT x13 ) ) ) OR ( x7 AND ( ( ( ( NOT x10 AND NOT x12 ) AND NOT x8 ) AND NOT x5 ) AND NOT x13 ) ) ) OR ( ( x5 AND ( x10 AND x13 ) ) AND ( ( NOT x12 AND NOT x8 ) AND NOT x7 ) ) ) OR ( ( x7 AND x13 ) AND ( ( ( NOT x10 AND NOT x12 ) AND NOT x8 ) AND NOT x5 ) ) ) OR NOT ( ( ( ( ( x10 OR x12 ) OR x8 ) OR x5 ) OR x7 ) OR x13 ) )
x10 = ( ( x12 AND NOT ( x2 AND ( x3 AND x14 ) ) ) OR ( x11 AND NOT ( x2 AND ( x3 AND x14 ) ) ) )
x11 = ( x12 OR ( ( x11 AND x4 ) AND NOT x10 ) )
x12 = ( x7 AND ( ( x5 AND NOT x10 ) OR NOT x13 ) )
x13 = ( ( ( x6 AND ( x10 OR NOT x5 ) ) AND NOT ( x13 AND ( x10 OR NOT x5 ) ) ) OR ( x11 AND ( x10 OR NOT x5 ) ) )
x14 = ( ( x11 AND NOT x1 ) OR ( ( x7 AND ( NOT x13 OR ( x5 AND NOT x10 ) ) ) AND NOT x1 ) ) \\
FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY & 15 & 0 & 15 & x1: v\_ADD, x2: v\_ATM, x3: v\_ATR, x4: v\_CHKREC, x5: v\_DSB\_, x6: v\_FAHRR, x7: v\_FANCD2I, x8: v\_FAcore, x9: v\_HRR2, x10: v\_ICL, x11: v\_NHEJ, x12: v\_NUC1, x13: v\_NUC2, x14: v\_TLS, x15: v\_p53 & x1 = ( ( ( x12 AND NOT x14 ) OR ( x13 AND NOT x14 ) ) OR ( ( x12 AND x13 ) AND NOT x14 ) )
x2 = ( ( x3 AND NOT ( x8 OR x4 ) ) OR ( x5 AND NOT ( x8 OR x4 ) ) )
x3 = ( ( x10 AND NOT x4 ) OR ( x2 AND NOT x4 ) )
x4 = ( ( ( ( ( x14 AND NOT x5 ) OR ( x9 AND NOT x5 ) ) OR ( x6 AND NOT x5 ) ) OR ( x11 AND NOT x5 ) ) OR NOT ( ( ( ( ( ( ( x10 OR x11 ) OR x6 ) OR x1 ) OR x4 ) OR x5 ) OR x9 ) OR x14 ) )
x5 = ( ( x12 AND NOT ( ( x6 OR x9 ) OR x11 ) ) OR ( x13 AND NOT ( ( x6 OR x9 ) OR x11 ) ) )
x6 = ( ( x7 AND x5 ) AND NOT ( x11 AND x4 ) )
x7 = ( ( x8 AND ( ( x5 AND ( x2 OR x3 ) ) OR ( x2 OR x3 ) ) ) AND NOT x4 )
x8 = ( ( x10 AND ( x2 OR x3 ) ) AND NOT x4 )
x9 = ( ( ( x14 AND ( x13 AND x5 ) ) AND NOT ( ( x11 OR x4 ) OR x6 ) ) OR ( ( x13 AND ( ( x10 AND x11 ) AND x5 ) ) AND NOT ( x4 OR x6 ) ) )
x10 = ( x10 AND NOT x5 )
x11 = ( ( x13 AND x5 ) AND NOT ( ( x9 OR x6 ) OR x4 ) )
x12 = ( x7 AND x10 )
x13 = ( ( ( x10 AND ( x2 OR x3 ) ) AND NOT ( x8 AND x7 ) ) OR ( ( x12 AND ( x10 AND x15 ) ) AND NOT ( x8 AND x7 ) ) )
x14 = ( ( ( x8 AND x1 ) AND NOT x4 ) OR ( x1 AND NOT x4 ) )
x15 = ( ( ( x11 AND NOT x4 ) OR ( x2 AND NOT x4 ) ) OR ( x3 AND NOT x4 ) ) \\
ROOT-STEM-CELL-2010 & 10 & 2 & 8 & x1: v\_ARF, x2: v\_AUXIAA, x3: v\_AUXIN, x4: v\_CLEX, x5: v\_JKD, x6: v\_MGP, x7: v\_PLT, x8: v\_SCR, x9: v\_SHR, x10: v\_WOX5 & x1 = NOT x2
x2 = NOT x3
x4 = ( x9 AND x4 )
x5 = ( x9 AND x8 )
x6 = ( ( x9 AND x8 ) AND NOT x10 )
x7 = x1
x8 = ( x9 AND x8 )
x10 = ( ( ( x1 AND x9 ) AND x8 ) AND NOT x4 ) \\
DROSOPHILA-NOTCH-PATHWAY & 13 & 6 & 7 & x1: v\_CtBP, x2: v\_Da, x3: v\_Delta, x4: v\_E\_Spl\_b1, x5: v\_E\_Spl\_b2, x6: v\_Emc, x7: v\_Gro, x8: v\_H, x9: v\_Mam, x10: v\_Nicd, x11: v\_Notch, x12: v\_Twi\_b1, x13: v\_Twi\_b2 & x4 = ( ( ( ( ( ( ( ( ( NOT x10 OR ( ( ( ( x10 AND NOT x4 ) AND NOT x8 ) AND NOT x7 ) AND NOT x1 ) ) OR ( ( ( ( ( x10 AND NOT x4 ) AND NOT x8 ) AND NOT x7 ) AND x1 ) AND NOT x9 ) ) OR ( ( ( ( x10 AND NOT x4 ) AND NOT x8 ) AND x7 ) AND NOT x9 ) ) OR ( ( ( x10 AND NOT x4 ) AND x8 ) AND NOT x9 ) ) OR ( ( ( ( ( x10 AND x4 ) AND NOT x5 ) AND NOT x8 ) AND NOT x7 ) AND NOT x1 ) ) OR ( ( ( ( ( ( x10 AND x4 ) AND NOT x5 ) AND NOT x8 ) AND NOT x7 ) AND x1 ) AND NOT x9 ) ) OR ( ( ( ( ( x10 AND x4 ) AND NOT x5 ) AND NOT x8 ) AND x7 ) AND NOT x9 ) ) OR ( ( ( ( x10 AND x4 ) AND NOT x5 ) AND x8 ) AND NOT x9 ) ) OR ( ( x10 AND x4 ) AND x5 ) )
x5 = ( ( ( ( ( x10 AND x4 ) AND NOT x8 ) AND NOT x7 ) AND NOT x1 ) AND x9 )
x6 = x10
x10 = x11
x11 = x3
x12 = ( ( ( ( ( ( ( ( ( NOT x6 AND NOT x2 ) AND x12 ) AND x13 ) OR ( NOT x6 AND x2 ) ) OR ( ( ( ( x6 AND NOT x4 ) AND NOT x2 ) AND x12 ) AND x13 ) ) OR ( ( x6 AND NOT x4 ) AND x2 ) ) OR ( ( ( ( ( x6 AND x4 ) AND NOT x5 ) AND NOT x2 ) AND x12 ) AND x13 ) ) OR ( ( ( x6 AND x4 ) AND NOT x5 ) AND x2 ) ) OR ( ( ( ( x6 AND x4 ) AND x5 ) AND x12 ) AND x13 ) )
x13 = ( ( ( NOT x6 AND x2 ) AND x12 ) OR ( ( ( x6 AND NOT x4 ) AND x2 ) AND x12 ) ) \\
FISSION-YEAST-2008 & 10 & 1 & 9 & x1: v\_Cdc25, x2: v\_Cdc2\_Cdc13, x3: v\_Cdc2\_Cdc13\_A, x4: v\_PP, x5: v\_Rum1, x6: v\_SK, x7: v\_Slp1, x8: v\_Start, x9: v\_Ste9, x10: v\_Wee1\_Mik1 & x1 = ( ( ( ( NOT x2 AND x1 ) AND NOT x4 ) OR ( ( x2 AND NOT x1 ) AND NOT x4 ) ) OR ( x2 AND x1 ) )
x2 = ( ( NOT x9 AND NOT x5 ) AND NOT x7 )
x3 = ( ( ( ( NOT x9 AND NOT x5 ) AND NOT x7 ) AND NOT x10 ) AND x1 )
x4 = x7
x5 = ( ( ( ( ( ( ( ( NOT x6 AND NOT x2 ) AND NOT x5 ) AND NOT x3 ) AND x4 ) OR ( ( ( NOT x6 AND NOT x2 ) AND x5 ) AND NOT x3 ) ) OR ( ( ( ( NOT x6 AND NOT x2 ) AND x5 ) AND x3 ) AND x4 ) ) OR ( ( ( ( NOT x6 AND x2 ) AND x5 ) AND NOT x3 ) AND x4 ) ) OR ( ( ( ( x6 AND NOT x2 ) AND x5 ) AND NOT x3 ) AND x4 ) )
x6 = x8
x7 = x3
x9 = ( ( ( ( ( ( ( ( NOT x6 AND NOT x2 ) AND NOT x9 ) AND NOT x3 ) AND x4 ) OR ( ( ( NOT x6 AND NOT x2 ) AND x9 ) AND NOT x3 ) ) OR ( ( ( ( NOT x6 AND NOT x2 ) AND x9 ) AND x3 ) AND x4 ) ) OR ( ( ( ( NOT x6 AND x2 ) AND x9 ) AND NOT x3 ) AND x4 ) ) OR ( ( ( ( x6 AND NOT x2 ) AND x9 ) AND NOT x3 ) AND x4 ) )
x10 = ( ( ( ( NOT x2 AND NOT x10 ) AND x4 ) OR ( NOT x2 AND x10 ) ) OR ( ( x2 AND x10 ) AND x4 ) ) \\
TRP-BIOSYNTHESIS & 6 & 1 & 5 & x1: v\_TrpE, x2: v\_TrpR, x3: v\_Trp\_b1, x4: v\_Trp\_b2, x5: v\_Trpext\_b1, x6: v\_Trpext\_b2 & x1 = ( NOT x3 AND NOT x2 )
x2 = ( x3 AND x4 )
x3 = ( ( ( ( ( NOT x5 AND NOT x3 ) AND x1 ) OR ( ( ( NOT x5 AND x3 ) AND NOT x4 ) AND x1 ) ) OR ( ( NOT x5 AND x3 ) AND x4 ) ) OR x5 )
x4 = ( ( x5 AND x6 ) AND x3 )
x6 = ( x5 AND x6 ) \\
MULTILEVEL-CELL-CYCLE & 13 & 1 & 12 & x1: v\_Cdc20, x2: v\_Cdh1, x3: v\_CycA, x4: v\_CycB, x5: v\_CycD, x6: v\_CycE, x7: v\_E2F, x8: v\_Rb\_b1, x9: v\_Rb\_b2, x10: v\_Skp2, x11: v\_UbcH10, x12: v\_p27\_b1, x13: v\_p27\_b2 & x1 = x4
x2 = ( ( ( ( NOT x3 AND NOT x4 ) OR ( ( NOT x3 AND x4 ) AND x12 ) ) OR ( ( ( x3 AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( x3 AND x12 ) AND x13 ) )
x3 = ( ( ( ( ( ( ( ( ( ( ( ( NOT x8 AND NOT x7 ) AND x3 ) AND NOT x1 ) AND NOT x2 ) OR ( ( ( ( ( NOT x8 AND NOT x7 ) AND x3 ) AND NOT x1 ) AND x2 ) AND NOT x11 ) ) OR ( ( ( ( NOT x8 AND NOT x7 ) AND x3 ) AND x1 ) AND NOT x11 ) ) OR ( ( ( NOT x8 AND x7 ) AND NOT x1 ) AND NOT x2 ) ) OR ( ( ( ( NOT x8 AND x7 ) AND NOT x1 ) AND x2 ) AND NOT x11 ) ) OR ( ( ( NOT x8 AND x7 ) AND x1 ) AND NOT x11 ) ) OR ( ( ( x8 AND x3 ) AND NOT x1 ) AND NOT x2 ) ) OR ( ( ( ( x8 AND x3 ) AND NOT x1 ) AND x2 ) AND NOT x11 ) ) OR ( ( ( x8 AND x3 ) AND x1 ) AND NOT x11 ) )
x4 = ( ( NOT x1 AND NOT x2 ) OR ( ( x1 AND NOT x2 ) AND NOT x11 ) )
x6 = ( ( NOT x8 AND x7 ) OR ( ( x8 AND NOT x9 ) AND x7 ) )
x7 = ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x8 AND NOT x3 ) AND NOT x4 ) OR ( ( ( NOT x8 AND NOT x3 ) AND x4 ) AND NOT x1 ) ) OR ( ( ( ( ( NOT x8 AND x3 ) AND NOT x4 ) AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( ( ( NOT x8 AND x3 ) AND NOT x4 ) AND x12 ) AND x13 ) ) OR ( ( ( ( ( ( NOT x8 AND x3 ) AND x4 ) AND x12 ) AND NOT x13 ) AND NOT x1 ) AND NOT x10 ) ) OR ( ( ( ( ( NOT x8 AND x3 ) AND x4 ) AND x12 ) AND x13 ) AND NOT x1 ) ) OR ( ( ( x8 AND NOT x9 ) AND NOT x3 ) AND NOT x4 ) ) OR ( ( ( ( x8 AND NOT x9 ) AND NOT x3 ) AND x4 ) AND NOT x1 ) ) OR ( ( ( ( ( ( x8 AND NOT x9 ) AND x3 ) AND NOT x4 ) AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( ( ( ( x8 AND NOT x9 ) AND x3 ) AND NOT x4 ) AND x12 ) AND x13 ) ) OR ( ( ( ( ( ( ( x8 AND NOT x9 ) AND x3 ) AND x4 ) AND x12 ) AND NOT x13 ) AND NOT x1 ) AND NOT x10 ) ) OR ( ( ( ( ( ( x8 AND NOT x9 ) AND x3 ) AND x4 ) AND x12 ) AND x13 ) AND NOT x1 ) )
x8 = ( ( ( ( ( ( ( ( ( ( ( NOT x8 AND NOT x6 ) AND NOT x3 ) AND NOT x4 ) OR ( ( ( ( NOT x8 AND NOT x6 ) AND NOT x3 ) AND x4 ) AND x12 ) ) OR ( ( ( NOT x8 AND NOT x6 ) AND x3 ) AND x12 ) ) OR ( ( NOT x8 AND x6 ) AND x12 ) ) OR ( ( ( ( x8 AND NOT x9 ) AND NOT x6 ) AND NOT x3 ) AND NOT x4 ) ) OR ( ( ( ( ( x8 AND NOT x9 ) AND NOT x6 ) AND NOT x3 ) AND x4 ) AND x12 ) ) OR ( ( ( ( x8 AND NOT x9 ) AND NOT x6 ) AND x3 ) AND x12 ) ) OR ( ( ( x8 AND NOT x9 ) AND x6 ) AND x12 ) ) OR ( x8 AND x9 ) )
x9 = ( ( ( ( ( ( ( ( NOT x5 AND x8 ) AND NOT x6 ) AND NOT x3 ) AND NOT x4 ) OR ( ( ( ( ( NOT x5 AND x8 ) AND NOT x6 ) AND NOT x3 ) AND x4 ) AND x12 ) ) OR ( ( ( ( NOT x5 AND x8 ) AND NOT x6 ) AND x3 ) AND x12 ) ) OR ( ( ( ( NOT x5 AND x8 ) AND x6 ) AND NOT x3 ) AND x12 ) ) OR ( ( ( ( ( NOT x5 AND x8 ) AND x6 ) AND x3 ) AND NOT x4 ) AND x12 ) )
x10 = ( ( NOT x8 OR ( x8 AND NOT x9 ) ) OR ( ( x8 AND x9 ) AND NOT x2 ) )
x11 = ( ( ( ( ( ( ( ( ( NOT x3 AND NOT x4 ) AND NOT x1 ) AND NOT x2 ) OR ( ( ( NOT x3 AND NOT x4 ) AND x1 ) AND NOT x2 ) ) OR ( ( ( ( NOT x3 AND NOT x4 ) AND x1 ) AND x2 ) AND x11 ) ) OR ( ( NOT x3 AND x4 ) AND NOT x2 ) ) OR ( ( ( NOT x3 AND x4 ) AND x2 ) AND x11 ) ) OR ( x3 AND NOT x2 ) ) OR ( ( x3 AND x2 ) AND x11 ) )
x12 = ( ( ( ( ( ( ( ( ( ( ( ( ( NOT x6 AND NOT x3 ) AND NOT x4 ) OR ( ( ( ( NOT x6 AND NOT x3 ) AND x4 ) AND NOT x12 ) AND NOT x10 ) ) OR ( ( ( ( ( NOT x6 AND NOT x3 ) AND x4 ) AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( ( ( NOT x6 AND NOT x3 ) AND x4 ) AND x12 ) AND x13 ) ) OR ( ( ( ( NOT x6 AND x3 ) AND NOT x4 ) AND NOT x12 ) AND NOT x10 ) ) OR ( ( ( NOT x6 AND x3 ) AND NOT x4 ) AND x12 ) ) OR ( ( ( ( NOT x6 AND x3 ) AND x4 ) AND NOT x12 ) AND NOT x10 ) ) OR ( ( ( ( ( NOT x6 AND x3 ) AND x4 ) AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( ( ( NOT x6 AND x3 ) AND x4 ) AND x12 ) AND x13 ) ) OR ( ( x6 AND NOT x12 ) AND NOT x10 ) ) OR ( ( ( x6 AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( x6 AND x12 ) AND x13 ) )
x13 = ( ( ( ( ( ( ( ( NOT x5 AND NOT x6 ) AND NOT x4 ) AND x12 ) OR ( ( ( ( NOT x5 AND NOT x6 ) AND x4 ) AND x12 ) AND NOT x10 ) ) OR ( ( ( ( ( ( NOT x5 AND x6 ) AND NOT x3 ) AND NOT x4 ) AND x12 ) AND NOT x13 ) AND NOT x10 ) ) OR ( ( ( ( ( NOT x5 AND x6 ) AND NOT x3 ) AND NOT x4 ) AND x12 ) AND x13 ) ) OR ( ( ( ( ( NOT x5 AND x6 ) AND NOT x3 ) AND x4 ) AND x12 ) AND NOT x10 ) ) OR ( ( ( ( NOT x5 AND x6 ) AND x3 ) AND x12 ) AND NOT x10 ) ) \\
ACUTE-RESPONSES-DURING-HYPERINSULINEMIA & 19 & 9 & 10 & x1: v\_FOXP3, x2: v\_GATA3, x3: v\_IFNG, x4: v\_IFNGe, x5: v\_IL10, x6: v\_IL10e, x7: v\_IL12e, x8: v\_IL2, x9: v\_IL21, x10: v\_IL21e, x11: v\_IL27e, x12: v\_IL2e, x13: v\_IL4, x14: v\_IL4e, x15: v\_INSULIN, x16: v\_RORGT, x17: v\_TBET, x18: v\_TGFB, x19: v\_TGFBe & x1 = ( ( x8 AND ( x18 OR x1 ) ) AND NOT ( x9 OR x16 ) )
x2 = ( ( ( x8 AND x13 ) OR x2 ) AND NOT ( ( ( x17 OR x18 ) OR x9 ) OR x3 ) )
x3 = ( ( x4 OR ( ( x3 OR x17 ) AND NOT ( x2 OR x18 ) ) ) AND NOT ( ( x9 OR x13 ) OR x5 ) )
x5 = ( x6 OR ( ( x5 AND ( ( ( ( x3 OR x9 ) OR x18 ) OR x2 ) OR x11 ) ) AND NOT x15 ) )
x8 = ( ( x12 OR ( x8 AND NOT x1 ) ) AND NOT ( ( x3 OR x9 ) OR ( x5 AND NOT x1 ) ) )
x9 = ( ( ( x10 OR x9 ) OR x16 ) AND NOT ( ( ( x3 OR x13 ) OR x5 ) OR x8 ) )
x13 = ( ( x14 OR ( ( x2 AND ( x8 OR x13 ) ) AND NOT x17 ) ) AND NOT ( x3 OR x9 ) )
x16 = ( ( x9 AND x18 ) AND NOT ( ( x17 OR x1 ) OR x2 ) )
x17 = ( ( ( x3 OR ( x7 AND NOT ( ( x9 OR x13 ) OR x5 ) ) ) OR x17 ) AND NOT ( ( x13 OR x2 ) OR x9 ) )
x18 = ( x19 OR ( ( x18 OR x1 ) AND NOT x9 ) ) \\
VEGF-PATHWAY-OF-DROSOPHILA & 18 & 8 & 10 & x1: v\_Aop, x2: v\_CNK, x3: v\_Drk, x4: v\_Dsor1, x5: v\_Ksr, x6: v\_Pnt, x7: v\_Pvf1, x8: v\_Pvf2, x9: v\_Pvf3, x10: v\_Pvr, x11: v\_Raf, x12: v\_Ras, x13: v\_Rl, x14: v\_Sos, x15: v\_Src42, x16: v\_Sty, x17: v\_Targets, x18: v\_msk & x1 = NOT x13
x3 = x10
x4 = x11
x6 = x13
x10 = ( ( x8 OR x7 ) OR x9 )
x11 = ( x12 AND ( ( x2 AND x5 ) AND x15 ) )
x12 = ( x14 AND NOT x16 )
x13 = ( x4 AND x18 )
x14 = x3
x17 = ( x6 AND NOT x1 ) \\
ERBB-REGULATED-G1-S-TRANSITION & 20 & 1 & 19 & x1: v\_AKT1, x2: v\_CDK2, x3: v\_CDK4, x4: v\_CDK6, x5: v\_CyclinD1, x6: v\_CyclinE1, x7: v\_EGF, x8: v\_ERBB1, x9: v\_ERBB1\_2, x10: v\_ERBB1\_3, x11: v\_ERBB2, x12: v\_ERBB2\_3, x13: v\_ERBB3, x14: v\_ERalpha, x15: v\_IGF1R, x16: v\_MEK1, x17: v\_MYC, x18: v\_p21, x19: v\_p27, x20: v\_pRB1 & x1 = ( ( ( ( ( ( ( ( NOT x15 AND NOT x8 ) AND NOT x12 ) AND NOT x9 ) AND x10 ) OR ( ( ( NOT x15 AND NOT x8 ) AND NOT x12 ) AND x9 ) ) OR ( ( NOT x15 AND NOT x8 ) AND x12 ) ) OR ( NOT x15 AND x8 ) ) OR x15 )
x2 = ( ( NOT x18 AND NOT x19 ) AND x6 )
x3 = ( ( NOT x18 AND x5 ) AND NOT x19 )
x4 = x5
x5 = ( ( ( ( NOT x16 AND x14 ) AND x1 ) AND x17 ) OR ( ( x16 AND x14 ) AND x17 ) )
x6 = x17
x8 = x7
x9 = ( x8 AND x11 )
x10 = ( x8 AND x13 )
x11 = x7
x12 = ( x11 AND x13 )
x13 = x7
x14 = ( ( NOT x16 AND x1 ) OR x16 )
x15 = ( ( ( NOT x14 AND x1 ) AND NOT x12 ) OR ( x14 AND NOT x12 ) )
x16 = ( ( ( ( ( ( ( ( NOT x15 AND NOT x8 ) AND NOT x12 ) AND NOT x9 ) AND x10 ) OR ( ( ( NOT x15 AND NOT x8 ) AND NOT x12 ) AND x9 ) ) OR ( ( NOT x15 AND NOT x8 ) AND x12 ) ) OR ( NOT x15 AND x8 ) ) OR x15 )
x17 = ( ( ( ( NOT x16 AND NOT x14 ) AND x1 ) OR ( NOT x16 AND x14 ) ) OR x16 )
x18 = ( ( NOT x3 AND NOT x1 ) AND NOT x17 )
x19 = ( ( ( NOT x3 AND NOT x2 ) AND NOT x1 ) AND NOT x17 )
x20 = ( x3 AND x4 ) \\
\bottomrule

\end{longtable}
% \end{adjustbox}



% \end{tabular}
% }

% \caption{Boolean‑network models used in this study.}
% \label{tab:bn-summary}
% \end{longtable}


\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/state_graphs_components/ASYMMETRIC-CELL-DIVISION-A_state_graph_components.png}
    \caption{Asymmetric Cell Division A}
\end{figure}




\clearpage
\section{Structured Causal Graph}
\label{appendix: causal_graph}


